GraFS: Graph Analytics Fusion and Synthesis

Graph analytics elicits insights from large graphs to inform critical decisions for business, safety and security. Several large-scale graph processing frameworks feature efficient runtime systems; however, they often provide programming models that are low-level and subtly different from each other. Therefore, end users can find implementation and specially optimization of graph analytics time-consuming and error-prone. This paper regards the abstract interface of the graph processing frameworks as the instruction set for graph analytics, and presents Grafs, a high-level declarative specification language for graph analytics and a synthesizer that automatically generates efficient code for five high-performance graph processing frameworks. It features novel semantics-preserving fusion transformations that optimize the specifications and reduce them to three primitives: reduction over paths, mapping over vertices and reduction over vertices. Reductions over paths are commonly calculated based on push or pull models that iteratively apply kernel functions at the vertices. This paper presents conditions, parametric in terms of the kernel functions, for the correctness and termination of the iterative models, and uses these conditions as specifications to automatically synthesize the kernel functions. Experimental results show that the generated code matches or outperforms hand-optimized code, and that fusion accelerates execution.

==> Extension.tex <==
\clearpage
\section{Specification and Fusion}

\subsection{Semantics}
\label{sec:semantics-app}
% \subsection{Language Semantics}

% \mclearpage
% \clearpage
% \begin{figure}
% \begin{figure}[t!]
% \begin{figure*}
% \begin{figure*}[t]
\begin{figure*}[h!]
% \begin{wrapfigure}[27]{R}{0.65\textwidth} 
% \vspace{-4ex}
\small

%    $
%    \begin{array}{c}
   \begin{mathpar}
% 
    \rulelabelp{SPRed}{SPRed}
    \inferrule[SPRed] {}{
%         \sem{P}(g) = \{\overline{p}\}
%     } {
        \sem{\underset{p \in P}{\R} \F(p)}\!(g)
        \ = \ 
%         \coloneqq
%         \underset{p \in \sem{P}(g)}{\R} \F(p)
%         \underset{p \in \sem{P}(g)}{\R} \F(p)
        \overline{
            \left[
                \v \mapsto
                \R \ \left\{\F(p) \ | \ p \in \sem{P}(g)(\v) \right\}
            \right]
        }_{
            \v \in \Vertices(g)
        }
    }

    \rulelabelp{SMBin}{SMBin}
    \inferrule[SMBin] {} {
        \sem{
            m \oplus m'
        }(g)
        \ = \ 
        \overline{
            \left[
                \v \mapsto
                \sem{m}(g)(\v) \oplus \sem{m'}(g)(\v)
            \right]
        }_{
            \v \in \Vertices(g)
        }        
    }

    \rulelabelp{SMLet}{SMLet}
    \inferrule[SMLet] {} {
        \sem{
            \ilet X \coloneqq M \lin e
        }(g)
        \ = \ 
%         e [X \mapsto \sem{M}]
        \overline{
%         \left[ \v \mapsto \sem{e \left[X \mapsto \sem{M}(g)(\v) \right]} \right]
        \left[ \v \mapsto \sem{e \left[X \coloneqq \sem{M}(g)(\v) \right]} \right]
%         \left[ \v \mapsto \sem{e \left[X \backslash \sem{M}(g)(\v) \right]} \right]
        }_{\v \in \Vertices(g)}
    }

    \rulelabelp{Var}{Var}
    \inferrule[Var] {} {
        \sem{
            x
        }(g)
        \ = \ 
        \bot
    }

    \rulelabelp{SVRed}{SVRed}
    \inferrule[SVRed] {}{
%         \mbox{for each $\v \in \Vertices(g)$: } 
%         \overline{\sem{m[v \mapsto \v]}\!(g) \ = \ n}_{\ \v \in \Vertices(g)}
%     } {
        \sem{
%             \underset{v \in \Vertices}{\R} m
            \underset{\Vertices}{\R} \ m
        }\!(g)
        \ = \ 
%         \R \ \{\overline{n}\}
        \R \ \left\{
%         \overline{
%             \overline{\sem{m[v \mapsto \v]}\!(g)}_{\ \v \in \Vertices(g)}
            \overline{\sem{m}\!(g)(\v)}_{\ \v \in \Vertices(g)}
%         }
        \right\}
    }

    \rulelabelp{SRBin}{SRBin}
    \inferrule[SRBin] {} {
        \sem{
            r \oplus r'
        }(g)
        \ = \ 
        \sem{r}(g) \oplus \sem{r'}(g)
    }

 
%         \sem{M} \ = \  
%         \sem{R[X' \mapsto]}
    \rulelabelp{SRLet}{SRLet}
    \inferrule[SRLet] {} {
        \sem{
            \begin{array}{l}
            \ilet X \coloneqq M \lin 
            \\
            \mlet X' \coloneqq E \lin
            \\
            \rlet X'' \coloneqq R \lin
            \\
            e
            \end{array}
        }(g)
        \ = \ 
        \sem{
        e
        \left[X'' \coloneqq
            \sem{R
                \left[X' \coloneqq
                    \left[ \overline{\v \mapsto \sem{E[X \coloneqq \sem{M}(g)(\v)]}} \right]
                    _{\v \in \Vertices(g)}
                \right]
            }\!(g)
        \right]
        }\!(g)
    }
     
    \rulelabelp{SPaths}{SPaths}
    \inferrule[SPaths] {} {
%     \rulelabelp{SPaths2}{SPaths2}
%     \inferrule[SPaths2] {} {
%         \sem{\Paths(\v)}(g) 
        \sem{\Paths}(g) 
        \ = \
        \overline{
            \left[
                \v \mapsto
%         \coloneqq
                \left\{ p \ | \ 
                    p \in \Paths(g) \land \tail(p) = \v %\sem{u}
%             \exists v' \in \Vertices(g). \ \path(p, v', v)
                \right\}
            \right]
        }_{
            \v \in \Vertices(g)
        }
%         \mbox{\ \ \ \ if \ \ \ \ }
% %         \sem{u} 
%         \v \in \Vertices(g)
    }

    {
    \rulelabelp{SArgsR}{SArgsR}
    \inferrule[SArgsR] {} {
        \sem{
            \underset{p \in P}{\mathsf{args}\,\R} \,\, \F(p)
        }(g)
        \ = \ 
%         \coloneqq
        \overline{
            \left[
                \v \mapsto
                \left\{p \ | \ p \in \{\overline{p}\} \land \F(p) = n \right\}
            \right]
        }_{
            \v \in \Vertices(g)
        }
        \mbox{\ \ \ \ where \ \ \ \ }
%         \underset{p \in \{\overline{p}\}}{\R} \F(p) = n
%         \\
%         p \in \{\overline{p}\}
%         \\
%         \F'(p) = n
    }
    \begin{array}{l}
        \{\overline{p}\} \ = \ \sem{P}(g)(\v)
        \\
%         \ \ \ \ 
        \R \in \{\min, \max\}
        \\
%         \ \ \ \ 
%         \\
        n = \R \ \left\{\F(p) \ | \ p \in \{\overline{p}\} \right\}
    \end{array}
    }

 
    \rulelabelp{SMPair}{SMPair}
    \inferrule[SMPair] {} {
        \sem{
            \<M, M'\>
        }(g)
        =
        \left\<\sem{M}\!(g), \sem{M'}\!(g)\right\>
    }    

    \rulelabelp{SMM}{SMM}
    \inferrule[SMM] {} {
        \sem{
            \R \ \F
        }(g)
        =
        \overline{
            \left[\v \mapsto 
                \R \ 
                \left\{ \F(p) \ | \ 
%                     p \in \sem{\Paths(\v)} 
                    p \in \sem{\Paths} 
                \right\}
            \right] 
        }_ {\v \in \Vertices(g)}
    }

    \rulelabelp{SRPair}{SRPair}
    \inferrule[SRPair] {} {
        \sem{
            \<R, R'\>
        }(g)
        =
        \left\<\sem{R}\!(g), \sem{R'}\!(g)\right\>
    }    

    \rulelabelp{SRR}{SRR}
    \inferrule[SRR] {} {
        \sem{
            \R \ 
            \left\< 
                \overline{[\v \mapsto n_\v]}_{\v \in \Vertices(g)},
                .., 
                \overline{[\v \mapsto n_\v']_{\v \in \Vertices(g)}}
            \right\>
        }\!(g)
        =
        \R \ \left\{
            \overline{
                \<n_\v, .., n_\v'\>
            }
            _{\v \in \Vertices(g)} 
        \right\}
    }

    \rulelabelp{SEBin}{SEBin}
    \inferrule[SEBin] {} {
        \sem{
            e \oplus e'
        }
%         (g)
        \ = \ 
%         \sem{e}(g) \oplus \sem{e'}(g)
        \sem{e} \oplus \sem{e'}
    }    

    \rulelabelp{SEVal}{SEVal}
    \inferrule[SEVal] {} {
        \sem{
            \n
        }
%         (g)
        \ = \ 
%         \sem{e}(g) \oplus \sem{e'}(g)
        \n
    }    

    \rulelabelp{SEM}{SEM}
    \inferrule[SEM] {} {
        \sem{
            d
        }
%         (g)
        \ = \ 
%         \sem{e}(g) \oplus \sem{e'}(g)
        d
    }    

    \rulelabelp{SEEPair}{SEEPair}
    \inferrule[SEEPair] {} {
        \sem{
            \<E, E'\>
        }
%         (g)
        =
%         \left\<\sem{E}\!(g), \sem{E'}\!(g)\right\>
        \left\<\sem{E}, \sem{E'}\right\>
    }    
% 
    \end{mathpar}
%     \end{array}
%     $

    \caption{\label{fig:semantics} 
        Denotational Semantics of the language presented in \autoref{fig:spec-lang}.
        The notation $\overline{[k_i \mapsto v_i]}_i$
        represents a finite map that maps each key $k_i$ to value $v_i$ over the range $i$.
        The notation $X \coloneqq V$ represents pointwise replacement of the variables $X$ with the values $V$.
%         Each rule defines the semantics of 
%         term constructors of specifications form \autoref{fig:spec-lang}.
    }

% \end{wrapfigure}
\end{figure*}
% \end{figure}



We now define a denotational semantics for the language that we presented in \autoref{fig:spec-lang}.
We present the semantics and prove that it is compositional.




The semantics is defined in \autoref{fig:semantics}. 
Given a graph $g$,
separate rules define
the semantics $\sem{}$ of each term constructor.
% is separately defined.
The semantics of an undefined or stuck computation is represented by $\bot$.
In each rule, 
if the conditions do not hold or 
the semantics of a subterm is $\bot$,
the semantics of the term is $\bot$.        
The semantics of term constructors with no rules is $\bot$ too.
For brevity, we elide the above pattern of undefined semantics
and present the defined semantics.






The semantics of $m$ terms are defined by
the rules \irule{SPRed}, \irule{SMBin}, \irule{SMLet} and \irule{Var}.
% 
The semantic domain $\D_m$ of $m$ 
% term 
% on a graph $g$ 
is a finite map
$\Vertices(g) \mapsto \Nat$ 
from each vertex of $g$ to natural numbers,
and
$\bot$.
% (for undefined).
% 
We use the notation $\overline{[k_i \mapsto v_i]}_i$
for a finite map that maps each key $k_i$ to value $v_i$ over the range $i$.
%
The rule \irule{SPRed} defines the
semantics of the reduction
$\underset{p \in P}{\R} \F(p)$
% in terms of 
using the semantics of the paths $P$.
It maps each vertex $\v$
to the reduction of the set of values resulting from applying $\F$ to the paths to $\v$.
% 
Since the reduction functions $\R$ (in the semantic domain) are commutative and associative,
they can be applied to any ordering of the set.
% 
The rule \irule{SMBin} defines the
the semantics of $m \oplus m'$ as
as the pointwise application of $\oplus$
to the semantics of $m$ and $m'$.
% 
% The same notation is used for 
Whether the notations $\R$ and $\oplus$ refer to the syntactic or semantic domains
is clear from the context.
They in the syntactic and semantic domains
when they are respectively on the left- and right-hand side of the rules.
% 
The rule \irule{SMLet} defines the
semantics of $\ilet X \coloneqq M \lin e$
as the pointwise substitution of 
the variables $X$ with the semantics of $M$
in $e$.
Pointwise substitution
replaces variables
with values
from a corresponding pair of structures.
(The formal definition of substitution is available in 
the appendix \autoref{sec:proofs-defs}).
% 
The rule \irule{Var} 
states that the semantics of free variables is undefined.





The semantics of $r$ terms is defined by
the rules \irule{SVRed}, \irule{SRBin}, and \irule{SRLet} and \irule{Var}.
% 
The domain $D_r$ of 
% a vertex-based computation 
$r$ 
% term 
% on a graph $g$ is 
is
the natural numbers $\Nat$ 
and 
$\bot$.
% (for undefined).
% 
The rule \irule{SVRed}
defines the semantics of the reduction
$\underset{\Vertices}{\R} \ m$
using the map resulted from the semantics of $m$;
it reduces the values of the 
% resulting 
map for 
% over 
all vertices.
% 
The rule \irule{SRBin} defines the semantics of
$r \oplus r'$ as the result of applying $\oplus$
to the semantics of $r$ and $r'$.
% 
The rule \irule{SRLet} defines the semantics of
triple-let terms
by three subsequent substitutions:
pointwise substitution of
the variables $X$ with
the semantics of $M$ in $E$,
substitution of
the variables $X'$ with
the semantics of $E$ in $R$,
and finally 
substitution of
the variables $X''$ with
the semantics of $R$ in $e$.


The semantics of paths $P$ is defined by the rules 
\irule{SPaths} and \irule{SArgsR}.
% 
The rule \irule{SPaths} defines the semantics of the term $\Paths$ as
a finite map from each vertex to the set of paths to the vertex.
% 
The rule \irule{SArgsR} defines the semantics of 
$\underset{p \in P}{\mathsf{args}\,\R} \,\, \F(p)$ where $\R$ is $\min$ or $\max$
using the map resulted from the semantics $\sem{P}$ of $P$;
it 
% defines a map that 
maps each vertex $\v$ to a subset of paths that $\sem{P}$ maps $v$ to:
the paths that their $\F$ value is the minimum or the maximum.
% result of applying 



The rules \irule{SMPair}, \irule{SRPair}, and \irule{SEEPair} define the semantics of 
pairs of $M$, $R$ and $E$ inductively.
%
The two rules 
\irule{SMM} 
and
\irule{SRR}
define the semantics of 
a single $M$ and 
a single $R$ respectively.
% 
The rule \irule{SMM} defines the semantics of
% of a single $M$
% of the form 
$\R \ \F$ that represents a path-based reduction.
It obtains the set of paths to each vertex from the semantics of $\Paths$,
and
% it 
maps each vertex $\v$
to the reduction of the set of values resulting from applying $\F$ to the paths to $\v$.
% 
The rule \irule{SRR} defines the semantics of 
% a single $R$
% of the form 
$\R \ 
\left\< \overline{[\v \mapsto n_\v]}_{\v \in \Vertices(g)},  .., \overline{[\v \mapsto n_\v']}_{\v \in \Vertices(g)}\right\>$
that represents the reduction of a tuple of maps over vertices;
it reduces 
the tuples 
% of the values of the maps 
$\<n_\v, .., n_\v'\>$
% for each vertex.
over 
% all 
vertices.
% 
The rules \irule{SEBin}, \irule{SEVal}, and \irule{SEM} define the semantics of expressions $e$.
For brevity, we assume that the operator $\oplus$ used in the rule \irule{SEBin} is overloaded for both numbers and maps in the semantic domain.



The semantics is compositional. 
If two terms are semantically equivalent,
replacing one with the other in any context is semantics-preserving.
Compositionality of the semantics is used to prove that
the fusion transformations are semantic-preserving.
% the soundness of the fusion transformations.
% semantics-preserving
The following theorem states that all the terms $r$, $m$, $M$ and $R$ are compositional.
The proofs are available in the appendix \autoref{sec:comp-proof}.

\begin{lemma}[Compositionality]
\label{lem:comp-app}
\ \\ \t
For all $r$, $r'$ and $\CR$,
if $\sem{r} = \sem{r'}$ then $\sem{\CR[r]} = \sem{\CR[r']}$.
\ \\ \t
For all $m$, $m'$, and $\CM$,
if $\sem{m} = \sem{m'}$ 
then
$\sem{\CM[m]} = \sem{\CM[m']}$.
\ \\ \t
For all $M$, $M'$, and $\CMs$,
if $\sem{M} = \sem{M'}$ 
then
$\sem{\CMs[M]} = \sem{\CMs[M']}$.
\ \\ \t
For all $R$, $R'$, and $\CRs$,
if $\sem{R} = \sem{R'}$ 
then
$\sem{\CRs[R]} = \sem{\CRs[R']}$.
\end{lemma}







\clearpage
\subsection{Language and Fusion Extensions}
\label{sec:ext-app}


In this section, we describe the language extensions and their corresponding fusion rules.
\autoref{fig:syntax-ext-app} represents the extensions to the syntax for the following subsections.


\begin{figure*}[h!]
\small

$
\begin{array}{rcll}

    r
        & \coloneqq &
        \boxed{\underset{\Vertices}{\R} \ m \oplus r}
        \ \ | \ \
        \boxed{\boxed{\underset{v \in \Vertices}{\R} m}}

%          \underset{\Vertices}{\R} \ m
%          \ \ | \ \
%          \!\circ r
         \ \ | \ \
         r \oplus r
         \ \ | \ \
         \dboxed{\circ \ r
         \ \ | \ \
        n}
        \ \ | \ \
%          v
%          \ \ | \ \
         &
         \mbox{Vertex-based Reduction}
%          \mbox{Specification}
    \\


        &&
        \ilet X \coloneqq M \lin
        &
%             \mbox{(or Vertex-based Reduction)}
        \\ &&
        \mlet X \coloneqq E \lin
        \\ &&
        \rlet X \coloneqq R \lin
        \\ &&
        e
% 
%         \xlet X \coloneqq R
%         \xlet \<\overline{x}\> \coloneqq
%         \<\overline{\underset{p \in P}{\R} F(p)}\>
%         \lin r
        \ \ | \ \ 
        x
    &
    \\

    m
        & \coloneqq &
         \underset{p \in P}{\R} F(p)
         \ \ | \ \ 
         m \oplus m
         \ \ | \ \ 
        &
        \mbox{Path-based Reduction}
        \\

    &&
        \boxed{\boxed{
            \ilet X \coloneqq M
            \lin v \ e
        }}
        \ \ | \ \ 
        x
    &
    \\


    P
        & \coloneqq &
%         &
        
%         \mbox{Set of Paths}
%     \\

%          & | &
%         \Paths(u', u)
%         \ \ | \ \
        \boxed{\boxed{
        \Paths(v)
        \ \ | \ \
        \Paths(v, v')
        }}
        \ \ | \ \
%         \underset{p \in P}{\mathsf{args}\,\A} \, \, F(p)
        \underset{p \in P}{\mathsf{args}\,\R} \, \, F(p)
%         \underset{p \in P}{\mathsf{args}\A} \ F(p)
%         \Paths(v, m)
        &
        \mbox{Paths}
    \\


    M
        & \coloneqq &
            \<M, M\>
            \ \ | \ \
%             m
            \boxed{\boxed{\underset{c}{\R} \ \F}}
        &
%             \mbox{Constant}
    \\


    \CR
        & \coloneqq &
        ...
        \ \ | \ \ 
%         \boxed{\underset{v \in \Vertices}{\R} m \oplus \CR}
        \boxed{\underset{\Vertices}{\R} \ m \oplus \CR}
        &
        \mbox{Context for $r$}
        \\


    v
        &  &
        &
        \mbox{Vertex Variable}
        \\

    s
        & \coloneqq &
%         &
            v
            \ \ | \ \
            \bot
        &
            \mbox{Source}
    \\

    o
        & \coloneqq &
%         &
            \rightarrow
            \ \ | \ \
            \leftarrow
        &
            \mbox{Orientation}
        \\


    c
        & \coloneqq &
%         &
            s
            \
            o
            \ \ | \ \
            \<c, c\>
        &
            \mbox{Path Configuration}
    \\


%     \multicolumn{4}{l}{\mbox{Definition of $e(v)$:}}
%     \\
%     
%     (e \oplus e')(v)
%         & \coloneqq &
%             e(v) \oplus e'(v)
%         &
%     \\
% 
%     x(v)
%         & \coloneqq &
%             x(v)
%         &
%     \\


    \R
        & \coloneqq &
            ...
            \ \ | \ \
            \dboxed{
            \union
            \ \ | \ \
            \intersect
            }
            &
            \mbox{Reduction Operation}
        \\

    \F
        & \coloneqq &
            ...
            \ \ | \ \ 
            \dboxed{
            \head
            \ \ | \ \
            \penultimate
            }
            &
            \mbox{Path Function}
%         \\

\end{array}
$

\caption{
    Extended Syntax.
    Dashed boxes for \autoref{sec:domain} and \autoref{sec:ext-app-unary-literal},
    solid boxes for \autoref{sec:multiple-rounds},
    and
    double solid boxes for \autoref{sec:vertex-var-app}
%     for Vertex Variables
}
\label{fig:syntax-ext-app}
\end{figure*}




\clearpage
% \subsubsection{Common Sub-expression Elimination}
\subsubsection{Common Operation Elimination}
\ \ \ 
% \subsubsection{Multiple Rounds}
\label{sec:com-subexp-elim}


\begin{figure*}[h!]
\small

\begin{mathpar}
\rulelabelp{IElim}{IElim}
\inferrule[IElim] {}{
\left(
{
\begin{array}{l}
\ilet \<X_1, X_2\> \coloneqq \<\R \ \F, \R \ \F\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
% \Rightarrow_r
\Rightarrow
\left(
{
\begin{array}{l}
\ilet X_1 \coloneqq \R \ \F \lin 
\\ 
\mlet X' \coloneqq E[X_2 \mapsto X_1] \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
}
 
\rulelabelp{ICom}{ICom}
\inferrule[ICom] {}{
\left(
{
\begin{array}{l}
\ilet \<X_1, X_2\> \coloneqq \<M_1, M_2\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
% \Rightarrow_r
\Rightarrow
\left(
{
\begin{array}{l}
\ilet \<X_2, X_1\> \coloneqq \<M_2, M_1\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
}

\rulelabelp{IAssL}{IAssL}
\inferrule[IAssL] {}{
\left(
{
\begin{array}{l}
\ilet \<X_1, \<X_2, X_3\>\> \coloneqq \<M_1, \<M_2, M_3\>\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
% \Rightarrow_r
\Rightarrow
\left(
{
\begin{array}{l}
\ilet \<\<X_1, X_2\>, X_3\> \coloneqq \<\<X_1, X_2\>, M_3\>\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
}

\rulelabelp{IAssR}{IAssR}
\inferrule[IAssR] {}{
\left(
{
\begin{array}{l}
\ilet \<\<X_1, X_2\>, X_3\> \coloneqq \<\<M_1, M_2\>, M_3\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
% \Rightarrow_r
\Rightarrow
\left(
{
\begin{array}{l}
\ilet \<X_1, \<X_2, X_3\>\> \coloneqq \<M_1, \<M_2, M_3\>\> \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
% \rlet X_2'' \coloneqq \underset{v \in \Vertices}{\R_3} \<x_1, x_2\> \lin
\rlet X'' \coloneqq R \lin
\\
e
\end{array}
}
\right)
}
% 
\end{mathpar}

\caption{
    Common Operation Elimination
}
\label{fig:fusion-rules-com-subexp-elim}
\end{figure*}


Fusion factors the path-based reduction, and vertex-based mappings and reductions.
The factoring facilitates common operation elimination.
For example, if a path-based reduction is calculated twice and assigned to two sets of variables, the extra calculation can be eliminated and the result of one calculation can be assigned to both sets of variables.



\autoref{fig:fusion-rules-com-subexp-elim} shows the elimination rules for path-based reductions.
The rule \irule{IElim} applies to adjacent similar path-based reductions.
The second reduction is eliminated. 
The variables for the second reduction are substituted with the variables for the first reduction.
To bring two path-based reductions adjacent to each other,
the rules \irule{ICom}, \irule{IAssL} and \irule{IAssR} state the commutativity and associativity properties of pairs of path-based reductions.



Similar eliminations can be applied to the factored vertex-based mappings in the second let and the factored vertex-based reductions in the third let.

As an example of common operation elimination,
see the fusion of the use-case \irule{DRR}
in \autoref{sec:example-fusions}.







\clearpage

% \subsection{Domain}
\subsubsection{Domain} 
\ \ \
\label{sec:domain}
% 


The scalar semantic domain of the core language was confined to the natural numbers.
The domain can be simply extended to booleans, vertex identifiers
and also sets of values.
The reduction operations are extended with union $\union$ and intersection $\intersect$
and
the path functions are extended with $\head$ and $\penultimate$.
The function $\head$ returns the identifier of the head vertex of the path and 
the function $\penultimate$ returns the identifier of the penultimate (that is the vertex before  the last) of the path.
These extensions are shown in dashed boxes in \autoref{fig:syntax-ext-app}



\subsubsection{Unary operations and Literals}
\ \ \ 
% \subsection{Unary operations and Literals}
\label{sec:ext-app-unary-literal}

\begin{figure*}[h!]
\small

\begin{mathpar}
% 
\rulelabelp{FILit}{FILit}
\inferrule[FILit]{}{
n
\ \ \ \    \Rightarrow   \ \ \ \
% \ilet \<\> \coloneqq \<\>
\ilet x \coloneqq \bot
\lin n
}
% 

\rulelabelp{FMVar}{FMLVar}
\inferrule[FMLVar]{}{
x
\ \ \ \    \Rightarrow   \ \ \ \
% \ilet \<\> \coloneqq \<\>
\ilet x' \coloneqq \bot
\lin x
}
% 
\\

\rulelabelp{FMPairp}{FMPair$'$}
\inferrule[FMPair$'$] {}{
\< X, x \>
\coloneqq
\<M, \bot \>
\ \ \ \    \rightarrow   \ \ \ \ 
X
\coloneqq
M
}

\rulelabelp{FMPairpp}{FMPair$''$}
\inferrule[FMPair$''$] {}{
\< x, X \>
\coloneqq   
\<\bot, M \>
\ \ \ \    \rightarrow   \ \ \ \ 
X
\coloneqq
M
}
% 
\\

\rulelabelp{FRLit}{FRLit}
\inferrule[FRLit] {}{
n
\ \ \ \    \Rightarrow   \ \ \ \ 
\!\!{
\begin{array}[t]{l}
\ilet x \coloneqq \bot \lin
\\ 
\mlet x' \coloneqq \bot \lin
\\ 
\rlet x'' \coloneqq \bot \lin
% \\
n
\end{array}}
}
% 
\\

\rulelabelp{FRPairp}{FRPair$'$}
\inferrule[FRPair$'$]{}{
\< X, x \>
\coloneqq
\<R, \bot \>
\ \ \ \    \rightarrow   \ \ \ \ 
X
\coloneqq
R
}

\rulelabelp{FRPairpp}{FRPair$''$}
\inferrule[FRPair$''$]{}{
\< x, X \>
\coloneqq
\<\bot, R \>
\ \ \ \    \rightarrow   \ \ \ \ 
X
\coloneqq
R
}
% 
\\

\rulelabelp{FIUni}{FIUni}
\inferrule[FIUni] {}{
\circ \ 
(\ilet X \coloneqq
% (\ilet \<\overline{x}\> \coloneqq
% \<\overline{\underset{p \in P}{\R} F(p)}\>
% \<\overline{m'}\>
M
% \lin m)
\lin e)
\ \ \ \    \Rightarrow   \ \ \ \ 
% \ilet \<\overline{x}\> \coloneqq
\ilet X \coloneqq
% \<\overline{\underset{p \in P}{\R} F(p)}\>
% \<\overline{m'}\>
M
% \lin \circ m
\lin \! \circ e
}


\rulelabelp{FRUni}{FRUni}
\inferrule[FRUni] {}{
\circ \ 
\left(
{\begin{array}{l}
\ilet X \coloneqq M \lin 
% \ilet X \coloneqq m \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
\rlet X'' \coloneqq R \lin
\\
e
\end{array}}
\right)
\ \ \ \    \Rightarrow   \ \ \ \ 
\left(
{\begin{array}{l}
\ilet X \coloneqq M \lin 
% \ilet X \coloneqq m \lin 
\\ 
\mlet X' \coloneqq E \lin
\\ 
\rlet X'' \coloneqq R \lin
\\
\circ \ e
\end{array}}
\right)
}
% 
\end{mathpar}

\caption{
    Extended Fusion Rules
    for Unary operators and constants
}
\label{fig:fusion-rules-unary-cons-app}
\end{figure*}



In this section, we present the fusion rules for the natural number literals $\n$ and unary operators $\circ$.
% 
As other rules 
% particularly the rules \irule{FILetBin} and \irule{FLetsBin}
expect terms to be in the let form,
the two rules \irule{FILit} and \irule{FRLit}
transform
a literal to dummy $m$ let and $r$ let forms.
% 
Since the two rules \irule{FMPair} and \irule{FRPair} 
apply to only non-$\bot$ reductions,
the rules \irule{FMPairp}, \irule{FMPairpp}, \irule{FRPairp} and \irule{FRPairpp}
remove the dummy $\bot$ reductions.
% 
The two rules \irule{FIUni} and \irule{FRUni}
simply apply the unary operator $\circ$ to the resulting expression $e$.




% Semantic rules:
% 
% \rulelabelp{SMUni}{SMUni}
% \inferrule[SMUni] {} {
%     \sem{
%         \circ \, m
%     }(g)
%     \ = \ 
%     \circ \, \sem{m}(g)
% }
% 
% 
% \rulelabelp{SVal}{SVal}
% \inferrule[SVal] {} {
%     \sem{
%         v
%     }(g)
%     \ = \ 
%     v
% }
% 
% \rulelabelp{SRUni}{SRUni}
% \inferrule[SRUni] {} {
%     \sem{
%         \circ \, r
%     }(g)
%     \ = \ 
%     \circ \, \sem{r}(g)
% }
% 
% \rulelabelp{SCon}{SCon}
% \inferrule[SCon] {} {
%     \sem{
%         v
%     }(g)
%     \ = \ 
%     v
% }
% 
% \rulelabelp{SEUni}{SEUni}
% \inferrule[SEUni] {} {
%     \sem{
%         \circ \, e
%     }(g)
%     \ = \ 
%     \circ \, \sem{e}(g)
% }
% 
% \rulelabelp{SBot}{SBot}
% \inferrule[SBot] {} {
%     \sem{
%         \bot
%     }(g)
%     =
%     \bot
% }









\clearpage
\subsubsection{Vertex Variables}
\ \ \ 
% \subsection{Vertex Variables}
\label{sec:vertex-var-app}

\begin{figure*}[h!]
\small

\begin{mathpar}
% 
\rulelabelp{FPRed-ext-app}{FPRed}
\inferrule[FPRed] {}{
\underset{p \in \Paths(v)}{\R} \F(p)
\\\\
\ \ \ \    \Rightarrow_m   \ \ \ \
\\\\
\ilet x \coloneqq
% \underset{p \in P}{\R} F(p)
\underset{\bot \rightarrow}{\R} \ \F
% \lin x(v)
\lin v \ x
% \lin x(u)
}

\rulelabelp{FPRedp-ext-app}{FPRed$'$}
\inferrule[FPRed$'$] {}{
\underset{p \in \Paths(v, v')}{\R} F(p)
\\\\
\ \ \ \    \Rightarrow_m   \ \ \ \
\\\\
\ilet x \coloneqq
\underset{v\rightarrow}{\R} \ \F
% \lin x(v')
\lin v' \ x
}

\rulelabelp{FPRedpp-ext-app}{FPRed$''$}
\inferrule[FPRed$''$] {}{
\underset{p \in \Paths(v, v')}{\R} \F(p)
\\\\
\ \ \ \    \Rightarrow_m   \ \ \ \
\\\\
\ilet x \coloneqq
\underset{v' \leftarrow}{\R} \ \F
% \lin x(v)
\lin v \ x
}

{\rulelabelp{FILetBin-ext-app}{FILetBin}
\inferrule[FILetBin] {}{
(\ilet
X_1
\coloneqq
M_1
\lin v \ e_1)
\ \oplus \ 
(\ilet
X_2
\coloneqq
M_2
% \lin e_2(v))
\lin v \ e_2)
\\\\
\ \ \ \    \Rightarrow_m   \ \ \ \ 
\\\\
\ilet \<X_1, X_2\> \coloneqq
\<M_1, M_2\>
% \lin e_1(v) \oplus e_2(v)
% \lin (e_1 \oplus e_2)(v)
\lin v \ (e_1 \oplus e_2)
}
\mbox{\ \ \ \ if }
{\begin{array}{l}
\free(e_1) \intersect X_2 = \emptyset   % \ \land
\\
\free(e_2) \intersect X_1 = \emptyset
\end{array}}
}

\begin{array}[t]{l}
\rulelabelp{FMPair-ext-app}{FMPair}
\inferrule[FMPair] {}{
% X \coloneqq
\left\<
% \underset{p \in P}{\R} F(p),
\underset{c}{\R} \ \F,
% \underset{p \in P}{\R'} F'(p)
\underset{c'}{\R'} \ \F'
\right\>
\ \ \ \    \Rightarrow_M   \ \ \ \ 
% X \coloneqq
% \underset{p \in P}{\R''} \, F''(p)
\underset{\<c, c'\>}{\R''} \ \F''
}
% \\ \mbox{\ \ \ \ where \ \ \ \ }
% \\ \mbox{where \ \ \ \ }
\\ \mbox{where \ \ }
f'' \coloneqq
\lambda p. \ \left\< F'(p), F(p) \right\>
% \\ \phantom{\mbox{where \ \ \ \ }}
\\ \phantom{\mbox{where \ \ }}
\R'' ( \<a, b\>, \<a', b'\> ) \coloneqq
\\ \phantom{\mbox{where \ \ }} \t
\left\<
\R (a, a'), \R' (b,  b') 
\right\>
\end{array}

\rulelabelp{FVRed-ext-app}{FVRed}
\inferrule[FVRed] {}{
\underset{v \in \Vertices}{\R} 
(\ilet X \coloneqq 
% \underset{c}{\R'} \, f \lin e(v))
\underset{c}{\R'} \, f \lin v \ e)
\ \ \ \    \Rightarrow_r   \ \ \ \ 
\!\!{
\begin{array}[t]{l}
\ilet X \coloneqq \underset{c}{\R'} \, f \lin 
\\
\mlet x \coloneqq e \lin
\\ 
\rlet x' \coloneqq \R \ x \lin
x'
\end{array}}
}
\end{mathpar}

\caption{
    Extended Fusion Rules
    for Vertex Variables
}
\label{fig:fusion-rules-ext-app}
\end{figure*}





The syntax of the core language
offers the simple term $\Paths$
that
does not specify the source and destination of paths.
Further, the vertex-based reduction 
$\underset{\Vertices}{\R} \ m$
does not bind a vertex variable.
% 
In this section, 
we extend the core syntax with 
path terms that can specify vertex variables as source and destination
and 
vertex-based reductions that can bind vertex variables.
We extend the fusion rules for the extended syntax.
 

In \autoref{fig:syntax-ext-app}, the double boxes shows
the extension to the core syntax presented in \autoref{fig:spec-lang}
to support vertex variables.
Only the changed or new non-terminals are shown
and the updated parts are boxed with solid lines.
% 
The extended vertex-based reduction
$\underset{v \in \Vertices}{\R} m$
binds the vertex variable $v$.
% 
The path constructors specify source and destination:
the term $\Paths(v)$ specifies the set of paths with any source and the destination $v$
and
the term $\Paths(v, v')$ specifies the set of paths with the source $v$ and the destination $v'$.
% 
In its simplest form, 
a factored path-based reduction
$M$
% $\underset{c}{\R} \ \F$
% $\R \ \F$
calculates
the reduction over 
paths from a source vertex $v$
to every destination vertex $v'$
and 
stores the result
in the destination vertices $v'$.
% 
It can also
calculate the reduction
over 
paths from every source vertex $v$
to a destination vertex $v'$
and
store the result
in the source vertices $v$.
% 
We call the vertex variable where the result is stored, the target vertex.
%
The let constructor 
$\ilet X \coloneqq M \lin v \ e$
of the path-based reductions $m$
carries 
the vertex $v$ that stores the result of the factored reduction $M$
with the expression $e$.
% 
% The terms $e(v)$ are simply defined as application of $v$ to every variable $x$ in $e$.
% 


The source $s$ of paths can be either a vertex $v$ or none $\bot$.
The orientation $o$ of paths is either forward $\rightarrow$ or backward $\leftarrow$.
% 
The configuration $c$ of paths is the pair of their source and orientation,
or a pair of other configurations.
% 
A single factored path-based reduction
$\underset{c}{\R} \ \F$
carries its configuration $c$.



\autoref{fig:fusion-rules-ext-app} shows the 
extension of the core fusion rules presented in
\autoref{fig:fusion-rules}.
% 
Only the updated fusion rules are shown.
% 
The rules \irule{FPRed-ext-app}, \irule{FPRedp-ext-app} and \irule{FPRedpp-ext-app}
convert 
path-based reductions over paths terms
% path terms 
to the let form.
The rule \irule{FPRed-ext-app}
converts
a path-based reduction over $\Paths(v)$
to
a let term 
with a factored path-based reduction that has no source $\bot$, forward orientation $\rightarrow$,
and
the target vertex $v$.
% 
The rules
\irule{FPRedp-ext-app} and \irule{FPRedpp-ext-app}
both convert
a path-based reduction over $\Paths(v, v')$
to let forms.
% 
The former stores the results in the destination vertices
and 
the latter stores the results in the source vertices.
% 
The former results in a let term with 
with a factored path-based reduction that has
source $v$, forward orientation $\rightarrow$,
and the target vertex $v'$.
The latter, on the other hand, results in a let term with 
a factored path-based reduction that has
source $v'$, backward orientation $\leftarrow$,
and the target vertex $v$.


The rule \irule{FILetBin-ext-app}
fuses 
an operation between
two path-based reductions in the let form to 
one.
% path-based reduction.
% 
The operation can be applied to the resulting expressions of the two let terms
only if they are stored in the same target vertex.
% 
Therefore,
the rule checks that
the explicit target vertex of the two let terms match.


The rule \irule{FMPair-ext-app}
simply passes 
% the target vertices and 
the configurations 
of the two reductions to the fused reduction.
 

A vertex-based reduction applies
a reduction 
to the results of a path-based reduction
over all vertices.
% Thus, the nested path-based reduction should store its results to the 
% 
The rule \irule{FVRed-ext-app} 
converts
the application of a vertex-based reduction to a path-based reduction
to the triple-let form;
% also checks that
% 
% The fusion rule will check that 
% This explicit variable $v$ in the let term
% is need to check that 
% 
it checks that
the vertex bound by the nesting vertex-based reduction
matches
the target vertex of the path-based reduction.


\clearpage
\subsubsection{Syntactic Sugar}
% \section{Syntactic Sugar}
\label{sec:syn-sugar-app}
\ \ \

\begin{figure*}[h!]
\small

$
% \!\!
{\begin{array}[t]{l}
\rulelabelp{FMRedP}{FMRed}
\inferrule[FMRed] {}{
\F \, (\underset{p \in P}{\mathsf{arg}\,\R} \,\, \F'(p))
% \ \ \ \    \Rightarrow_m   \ \ \ \
\ \ \ \    \coloneqq   \ \ \ \
% \underset{p \in P}{\R'} \, \<\F'(p), \F(p)\>
\ilet \<x, x'\> \coloneqq \underset{p \in P}{\R'} \, \F''(p) \lin x'
}
\mbox{\ \ \ \ where \ \ \ \ }
\R \in \{\min, \max\}
\\
\F'' \ \coloneqq \ 
\lambda p. \ \<\F'(p), \F(p)\>
\\
\R' ( \<a, b\>, \<a', b'\>) \ \coloneqq \ 
% \\\t
% \lif \ (a' = a) \ \<a, b\> \ 
% \\
% \lelse \ 
\lif \ (\R (a, a') = a) \lthen \<a, b\> \ 
% \\\t
% \phantom{\lelse \ }
\lelse \ \<a', b'\>
\end{array}
}
$

\ \\
\ \\

$
\begin{array}{cc}
% \begin{array}[t]{l}
\begin{array}{l}
% \begin{array}[t]{rcl}
% \multicolumn{3}{l}{
% \mbox{Syntactic sugar for $m$:}
% }
% \\
\rulelabelp{PSize}{PSize}
\inferrule[PSize] {}{
    |P|
%     & \coloneqq &
    \ \ \ \    \coloneqq   \ \ \ \
    \displaystyle
    \sum_{p \in P} 1
}
\\
\rulelabelp{ROp}{ROp}
\inferrule[ROp] {}{
%     \underset{v \in \{\overline{v}\}}{\R} m
    \underset{v \in \{\v_1, .., v_n\}}{\R} m
%     & \coloneqq &
    \ \ \ \    \coloneqq   \ \ \ \
    ((m[v \coloneqq v_1] \ \R \ m[v \coloneqq v_2]) \ \R \ .. \ m[v \coloneqq v_n])
}
\end{array}

&

% \begin{array}[t]{rcl}
% \multicolumn{3}{l}{
% \mbox{Syntactic sugar for $r$:}
% }
% \\
\rulelabelp{VSel}{VSel}
\inferrule[VSel] {}{
    {\begin{array}{l}
    \underset{v \in \Vertices \, \land \, m'}{\R} m
%     & \coloneqq &
    \ \ \ \    \coloneqq   \ \ \ \
    \underset{v \in \Vertices}{\R'} \<m', m\> 
    \\
    \mbox{where \ \ \ \ }
    \R' (b, \<a', b'\>) \coloneqq
    \\ \phantom{\mbox{where \ \ \ \ }} \t
    \lif \ (a') \lthen \R(b, b')
    \\ \phantom{\mbox{where \ \ \ \ }} \t
    \lelse \ b
    \end{array}}
}
% \end{array}
\end{array}
$

\caption{
    Syntactic Sugar
}
\label{fig:syntactic-sugar}
\end{figure*}


Syntactic sugar enable concise specifications.
In \autoref{fig:syntactic-sugar}, 
we present the syntactic sugar and the rules that desugar them.


The term
$\F (\underset{p \in P}{\mathsf{arg}\,\R} \,\, \F'(p))$
where $\R$ is either $\min$ or $\max$
first finds a path $p$ in $P$ with the minimum or maximum value for the function $\F'$
and then returns the result of applying $\F$ to $p$.
% 
It is used to specify the \irule{BFS} use-case.
% 
The rule \irule{FMRedP} expands this term to
% This term can be simply replaced with
a path-based reduction 
% $m$ term
in the let form
$\ilet \<x, x'\> \coloneqq \underset{p \in P}{\R'} \, \F''(p) \lin x'$.
The path function $\F''$ returns the pair of the results of $\F'$ and $\F$.
The reduction function $\R'$ returns 
the input pair with the minimum or maximum first element.
 

The term $|P|$ specifies the size of the set of paths $P$.
% It is used to specify the \irule{NP} and \irule{NSP} use-cases.
It is used to specify the \irule{NSP} use-case.
The rule \irule{PSize} simply expands it to 
the path-based reduction 
% $\displaystyle \sum_{p \in P} 1$
$\underset{p \in P}{\sum} 1$
that counts the number of paths.




The term 
% $\underset{v \in \{\overline{v}\}}{\R} m$
$\underset{v \in \{v_1, .., v_n\}}{\R} m$
is a vertex-based reduction over a limited set of vertices 
% $\{\overline{v}\}$.
$\{v_1, .., v_n\}$.
It is used to specify the \irule{Radius} use-case.
The rule \irule{ROp} expands this term to 
operations between to path-based reductions $m[v \coloneqq v_i], i\in\{1..n\}$.
The operation corresponds to the reduction function $\R$;
for example, the reduction function $\sum$ is unrolled to the operation $+$.



The term
$\underset{v \in \Vertices \, \land \, m'}{\R} m$
specifies a vertex-based reduction of $m$ over 
the selected vertices $v$
% for which the result of $m'$ is true.
for which $m'$ evaluates to true.
This idiom was used to specify the $\DS$ use-case.
The rule \irule{VSel} expands it to 
the path-based reduction
$\underset{v \in \Vertices}{\R'} \<m', m\>$.
% 
The path-based reduction calculates a pair of values for $m'$ and $m$ at every vertex.
Then, the vertex-based reduction
starts with the none value $\bot$ and
iteratively applies $\R'$ to 
the current value and the pair value of each vertex.
Given an input pair, the function $\R'$
applies the reduction $\R$
to the second element
only if the first element is true.
Thus, the reduction $\R'$ filters 
vertices for which $m'$ evaluates to false.





\clearpage
% \subsection{Multiple Rounds}
\subsubsection{Nested Triple-lets}
\ \ \ 
% \subsubsection{Multiple Rounds}
\label{sec:multiple-rounds}


\begin{figure*}[h!]
\small

\begin{mathpar}
% 
\rulelabelp{FRR}{FRR}
\inferrule[FRR] {
% X
% \coloneqq
r_1
\ \ \ \    \Rightarrow_r   \ \ \ \ 
% X'
% \coloneqq
r_2
}{
\CR[r_1]
\ \ \ \    \Rightarrow_r   \ \ \ \ 
\CR[r_2]
}
% 
% 
% \rulelabelp{RLet}{RLet}
% \inferrule[RLet] {}{
% \underset{\Vertices}{\R} \ m \oplus r
% \\\\
% \ \ \ \    \Rightarrow_r   \ \ \ \
% \\\\
% \xlet x \coloneqq r \lin 
% % \\\\
% \underset{\Vertices}{\R} \ m \oplus x
% }
% 
\end{mathpar}

\caption{
    Extended Fusion Rules
    for Multiple Rounds
}
\label{fig:fusion-rules-ext-mround-app}
\end{figure*}





The core syntax supports expressions that can be fused to 
a single iteration-map-reduce triple-let term.
% 
In this subsection, 
we extend the core syntax 
to support nested vertex-based reductions,
and extend the fusion rules 
to fuse nested reductions.
% 
% to support expressions 
% that are fused to 
% % a sequence of iteration-map-reduce 
% nested triple-let terms.
% % The sequence of multiple 
% 
Nested triple-let terms that are closed (i.e.\ do not have free variables)
can be factored out.
% 
Thus,
nested triple-let terms
can be
translated to a sequence of
% multiple
iteration-map-reduce
rounds 
% of computation 
on the graph.
% 
% 
% Independent 
% Nested 
% triple-let terms translate to a sequence of
% % multiple
% iteration-map-reduce
% rounds 
% % of computation 
% on the graph.


In \autoref{fig:syntax-ext-app}, 
the single boxes show
the extensions to the core syntax presented in \autoref{fig:spec-lang}
to support multiple rounds.
% 
The constructors of vertex-based reductions $r$ include the new term
$\underset{\Vertices}{\R} \ m \oplus r$
where 
an operation $\oplus$ can be applied to a path-based reduction $m$ and a nested vertex-based reduction $r$.
This nested $r$ leads to a round of iteration-map-reduce.
Similarly,
the vertex-based reduction contexts $\CR$ include the term
$\underset{\Vertices}{\R} \ m \oplus \CR$
so that 
the nested vertex-based reductions can be fused as well.
% 
As \autoref{fig:fusion-rules-ext-mround-app} shows,
the fusion rules are extended by the rule \irule{FRR} to allow the fusion of nested vertex-based reductions.




% The core language supports only expressions that can be fused to one round of iteration-map-reduce.
% However, path-based reductions $m$ may use nested vertex-based reductions $r$.
For example, consider the following use-case $\RDS$ that calculates
the capacity of narrowest path to the nodes that fall out of the radius from the node $s$.

$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet 
        \SP \coloneqq \lambda s, v. \ 
        \displaystyle \min_{  p \in \Paths(s, v) } \weight(p) 
    \lin
    \\
    & &
    \llet 
        \NP \coloneqq \lambda s, v. \ 
        \displaystyle \min_{  p \in \Paths(s, v) } \capacity(p)
    \lin
    \\
    & &
    \displaystyle
    \min_{
        v \in \Vertices \, \land \,
        \displaystyle
        \SP(s, v)
        < \Radius
    }
    \NP(s, v)
\end{array}
$$

Unrolling the let terms results in the following:

$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \displaystyle
    \min_{
        v \in \Vertices \, \land \,
        \displaystyle
        \left(
        \min_{  p \in \Paths(s, v) }
        \weight(p)
        \right)
        < \Radius
    }
    \left(
    \displaystyle \min_{  p \in \Paths(s, v) } \capacity(p)
    \right)
\end{array}
$$

By the rule \irule{VSel}, this specification is desugared to the following:

$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \displaystyle
    \underset{v \in \Vertices}{\R}
    \ \ 
    \left\<
        \left(
        \min_{  p \in \Paths(s, v) }
        \weight(p)
        \right) < 
        \Radius,
        \left(
        \displaystyle \min_{  p \in \Paths(s, v) } \capacity(p)
        \right) 
    \right\>
    \\
    \\
    & &    
    \mbox{where \ \ \ \ }
    \R (b, \<a', b'\>) \coloneqq
    \\ & & \phantom{\mbox{where \ \ \ \ }} \t
    \lif \ (a') \lthen \min(b, b')
    \\ & & \phantom{\mbox{where \ \ \ \ }} \t
    \lelse \ b
\end{array}
$$



We note that in the above specification,
the path-based reduction
$\SP(s, v) < \Radius$
includes
the nested vertex-based reduction
$\Radius$.
% 
From \autoref{fig:radius-fusion}, $\Radius$ can be fused to following:

$$
\Radius \ = \
\left(
\begin{array}{l}
\ilet \<x, y\> \coloneqq 
    \underset{\<s_1, s_2\>}{\R'} \ \F
    \lin
\\ 
\mlet \<x', y'\> \coloneqq \<x, y\> \lin
\\ 
\rlet \<x'', y''\> \coloneqq 
%     \underset{v \in \Vertices}{\R'} \ \< x',  y' \>
    \R'' \ \< x',  y' \>
    \lin
\\
\min(x'', y'')
\end{array}
\right)
\mbox{\ \ where \ \ }
\begin{array}{l}
\F \coloneqq \lambda p. \ \left\< \length(p), \length(p) \right\> 
\\
\R' \, ( \<a, b\>, \<a', b'\> ) \coloneqq
\\ \t
\left\<
\min (a, a'), \min (b,  b') 
\right\>
\\
\R'' \, ( \<a, b\>, \<a', b'\> ) \coloneqq
\\ \t
\<\max (a, a'), \max (b,  b') \>
\end{array}
$$

Therefore, The rules \irule{FRR} can be used to fuse the nested $\Radius$ term to the above triple-let term.
Then, since $\Radius$ is a closed term, it can be factored out as a let term.
Thus, $\RDS$ can be rewritten as follows:


$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet \mathit{radius} :=     
    \left(
    \begin{array}{l}
    \ilet \<x, y\> \coloneqq 
        \underset{\<s_1, s_2\>}{\R'} \ \F
        \lin
    \\ 
    \mlet \<x', y'\> \coloneqq \<x, y\> \lin
    \\ 
    \rlet \<x'', y''\> \coloneqq 
    %     \underset{v \in \Vertices}{\R'} \ \< x',  y' \>
        \R'' \ \< x',  y' \>
        \lin
    \\
    \min(x'', y'')
    \end{array}
    \right) \lin
    \\
    & &
    \underset{v \in \Vertices}{\R}
    \ \ 
    \left\<
        \left(
        \displaystyle 
        \min_{  p \in \Paths(s, v) }
        \weight(p)
        \right) < 
        \mathit{radius},
        \left(
        \displaystyle \min_{  p \in \Paths(s, v) } \capacity(p)
        \right) 
    \right\>
\end{array}
$$

By the rule \irule{FPRed} (and then for the first element of the pair, the rules \irule{FMVar}, \irule{FILetBin} and \irule{FMPairp}), it can be fused to the following:

$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet \mathit{radius} \coloneqq
    \left(
    \begin{array}{l}
    \ilet \<x, y\> \coloneqq 
        \underset{\<s_1, s_2\>}{\R'} \ \F
        \lin
    \\ 
    \mlet \<x', y'\> \coloneqq \<x, y\> \lin
    \\ 
    \rlet \<x'', y''\> \coloneqq 
        \R'' \ \< x',  y' \>
        \lin
    \\
    \min(x'', y'')
    \end{array}
    \right) \lin
    \\
    & &
    \underset{v \in \Vertices}{\R}
    \ \ 
    \left\<
        \ilet x \coloneqq
        \underset{s}{\min} \ \weight
        \lin x < \mathit{radius},
        \ \ 
        \ilet y \coloneqq
        \underset{s}{\min} \ \capacity
        \lin y
    \right\>
\end{array}
$$

By the rule \irule{FILetBin},
it is fused to the following:

$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet \mathit{radius} \coloneqq
    \left(
    \begin{array}{l}
    \ilet \<x, y\> \coloneqq 
        \underset{\<s_1, s_2\>}{\R'} \ \F
        \lin
    \\ 
    \mlet \<x', y'\> \coloneqq \<x, y\> \lin
    \\ 
    \rlet \<x'', y''\> \coloneqq 
        \R'' \ \< x',  y' \>
        \lin
    \\
    \min(x'', y'')
    \end{array}
    \right) \lin
    \\
    & &
    \underset{v \in \Vertices}{\R}
    \ \
        \left(
        \ilet \<x, y\> \coloneqq
        \<
            \underset{s}{\min} \ \weight,
            \underset{s}{\min} \ \capacity
        \>
        \lin \<x < \mathit{radius}, y\>
        \right)
\end{array}
$$

By the rule \irule{FMPair},
it is fused to the following:


$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet \mathit{radius} \coloneqq
    \left(
    \begin{array}{l}
    \ilet \<x, y\> \coloneqq 
        \underset{\<s_1, s_2\>}{\R'} \ \F
        \lin
    \\ 
    \mlet \<x', y'\> \coloneqq \<x, y\> \lin
    \\ 
    \rlet \<x'', y''\> \coloneqq 
        \R'' \ \< x',  y' \>
        \lin
    \\
    \min(x'', y'')
    \end{array}
    \right) \lin
    \\
    & &
    \underset{v \in \Vertices}{\R}
    \ \
        \left(
        \ilet \<x, y\> \coloneqq
            \underset{\<s, s\>}{\R'''} \ \F'
        \lin \<x < \mathit{radius}, y\>
        \right)
\\
\\ && \mbox{where \ \ }
\F' \coloneqq
\lambda p. \ \left\< \weight(p), \capacity'(p) \right\>
\\ && \phantom{\mbox{where \ \ }}
\R''' ( \<a, b\>, \<a', b'\> ) \coloneqq
\\ && \phantom{\mbox{where \ \ }} \t
\left\<
\min (a, a'), \min (b,  b') 
\right\>
\end{array}
$$


By the rule \irule{FVRed},
it is fused to the following:


$$
\begin{array}{rcl}
    \RDS(s) 
    & = &
    \llet \mathit{radius} \coloneqq
    \left(
    \begin{array}{l}
    \ilet \<x, y\> \coloneqq 
        \underset{\<s_1, s_2\>}{\R'} \ \F
        \lin
    \\ 
    \mlet \<x', y'\> \coloneqq \<x, y\> \lin
    \\ 
    \rlet \<x'', y''\> \coloneqq 
        \R'' \ \< x',  y' \>
        \lin
    \\
    \min(x'', y'')
    \end{array}
    \right) \lin
    \\
    & &
    \left(
    {\begin{array}{l}
    \ilet \<x, y\> \coloneqq 
%     \R'' \ \< x',  y' \> \lin 
    \underset{\<s, s\>}{\R''} \ \F'
    \\ 
    \mlet \<x', y'\> \coloneqq  \lin \<x < \mathit{radius}, y\>
    \\ 
    \rlet x'' \coloneqq \R \  \<x', y'\> \lin
    \\
    x''
    \end{array}}
    \right)    
\end{array}
$$


The above specification is the sequence of two iteration-map-reduce triple let terms.







% \clearpage
% \subsubsection{Non-Path-Based Algorithms}
% \ \ \ 
% % \vspace{.5cm}
% % \begin{wrapfigure}{R}{.5\textwidth}
% \begin{figure}[h!]
% \small
% \centering
% $
% \begin{array}{rcll}
%     f(v)
%         & \coloneqq &
% %         \boxed{
%          \underset{(u, v) \in E}{\R} e
%          \ \ | \ \ 
%          i \oplus e
% %          \ \ | \ \ 
%          %}
%         &
%         \mbox{Reduction}
%         \\
%         
% %     i
% %         & \coloneqq &
% %         \boxed{
% %          \underset{e \in E}{\R} \lambda n,e. x
% %          \ \ | \ \ 
% %          i \oplus e
% %          \ \ | \ \ 
% %          }
% %         &
% %         \mbox{Edge-based Reduction}
% %         \\
% 
% 
%     E
%         & \coloneqq &
% %         &
%         
% %         \mbox{Set of Paths}
% %     \\
% 
% %          & | &
% %         \Paths(u', u)
% %         \ \ | \ \
% %         \boxed{
%         \mathsf{InEdges}(v)
%         %  \mathsf{OutEdges}(v)
% %         }
%         &
%         \mbox{Edges}
%         \\
% 
% 
%     e
%         & \coloneqq &
%         e \oplus e
%          \ \ | \ \
% %         &
% %         \mbox{Set of Paths}
% %     \\
% 
% %          & | &
% %         \Paths(u', u)
% %         \ \ | \ \
% %         \boxed{
%         \mathsf{indeg}(v)
%         \ \ | \ \
%         \mathsf{outdeg}(v)
%         \ \ | \ \
%         f(e)
%         \ \ | \ \
%         v
%         \ \ | \ \
%         c
% %         }
%         &
%         \mbox{Expression}
%        
% \end{array}
% $
% 
% \caption{
%     Extended Syntax 
%     for Non-Path-Based Computations
% }
% \label{fig:syntax-ext-non-path}
% % \end{wrapfigure}
% \end{figure}
% 
% 
% There are another class of graph algorithms which can be specified in $\name$ with minor extensions.
% The specification of this class of algorithms applies a reduction function
% R to the result of an edge function $\lambda \S,e. x$. We saw that the path-based computations can be
% calculated using local propagation at vertex-level. 
% The edge function $\lambda \S,e. x$ in edge-based computations is the propagate function $\P$ itself.
% We present the specification of such computations in \autoref{def:spec-iter-non-path}.
% The synthesis is based on the method proposed in the \cite{zhang2012accelerate}. 
% The idea is to break the iterative computation into accumulative updates.
% The accumulative updates can be easily mapped to the frameworks.
% 
% \begin{definition}[Specification]~\\
% \label{def:spec-iter-non-path}
% $
% \Spec(v) = 
% \R_{ e \, \in \, \{e \, | \, e \in \mathsf{incoming}(v) \; \land \; \C(e) \} } \ \lambda \Spec(\mathsf{source}(e)), e. x)
% $
% \end{definition}
% The correctness conditions for iterative accumulative updates are as follows:
% \begin{itemize}
% \item All the properties for the $\R$ mentioned before for path-based computations.
% \item The propagate function must be distributive with respect to the reduction operation $\R$.
% Formally, the following condition must hold on the propagate function:
% \end{itemize}
% 
% $
% \begin{array}{l}
% \forall v_1, v_2, e. \ 
% % \\ \t\t\t
% % \C(p_1) \land \C(p_2) \ \land
% \\ \t\t\t 
% \llet \P \coloneqq \lambda n,e. x \lin
% \\ \t\t\t
% \P\left[
%     \R(v_1, v_2), \ 
%        e 
% \right] = 
% \R\left[
%     \P(v_1, e), \ 
%     \P(v_2, e)
% \right]
% \end{array}
% $
% 
% We present the extension of the syntax in \autoref{fig:syntax-ext-non-path}.
% The rule $i$ captures the iterative edge-based computation which applies reduction function $\R$
% to the result of an edge function. Binary operators can also be applied to the result of edge-based computations and
% any free expressions ($i \oplus e$).
% %In general, $\name$ can synthesize any algorithm from it's vertex calculation.
% 
% 
% 
% 
% \textbf{Pagerank. \ }
% Pagerank is an iterative algorithm used for ranking the nodes of the graph based on the authority of the
% nodes. A node is considered more authoritative if it has higher rank. Therefore, the more the score of 
% the predecessors of a node is, the higher the node's pagerank score.
% We can define the pagerank algorithm by specifying the computation 
% at vertex level and the $\name$ tool generates the code for the 
% % four 
% five
% mentioned framework.
% 
% $
% \begin{array}{rclr}
%             PR(v)& = & % \{
%            \displaystyle \sum_{(u, v) \in \mathsf{InEdges(v)}} d \times \frac{PR(u)}{\mathsf{outdeg}(u)} + (1-d)
%            &
%            \mbox{PageRank}
% %             \\
% %             \\
% %             \I & \coloneqq &
% %                 \lambda v. \ \ 
% %                 1 \, / \, |V|
% %             \\
% %             \P & \coloneqq &
% %                 \lambda n, e. \ \ 
% %                 n \, / \, \mathsf{outdeg}(\mathsf{src}(e))
% %             \\
% %             \R & \coloneqq &
% %             +
% %             \\
% %             \M & \coloneqq &
% %                 \lambda n, v. \ \ 
% %                 \gamma * n \, + \, (1-\gamma) / |V|
% %             \\
% %             \\
% \end{array}
% $
% 
% We can break the PageRank computation into two phases. First, at each vertex we calculate the 
% first expression, $d\sum_{uv \in \mathsf{InEdges}(v)} \frac{PR(u)}{deg(u)}$. Second, we add the remaining value to the PageRank, $1-d$.
% 
% 
% \textbf{Linear Equation (Jacobi Method). \ }
% We can specify the system of linear equations in terms of an iterative computation over a weighted graph.
% $AX = B$ represents the linear equation.
% Typically, the matrix $A$ is a $v \times v$ matrix storing the coefficient of the equations and 
% matrix $B$ stores the constant values of the equation.
% However, in the graph representation, the coefficient of the equations (except coefficients on the 
% diagonal of the matrix $A$)
% are stored as weights on the corresponding edges.
% We store the diagonal coefficients of the initial matrix $A_{v \times v}$ in a separate matrix $A'_{v \times 1}$.
% $X$ is the solution to the equation.
% 
% 
% $
% \mbox{Let $A'$ and $B$ be constant matrices of size $v \times 1$ in}\\[.5em]
% \begin{array}{rclr}
%             X(v)
%             & = & % \{
%            \displaystyle \sum_{(u,v) \in \mathsf{InEdges}(v)} -\frac{w_{uv} \times X(u)}{A'_{v}} + \frac{B_v}{A'_{v}}
%            &
%            \mbox{Jacobi Method}
% \end{array}
% $
% 
% 
% \textbf{Co-Training Expectation Maximization. \ }
% 
% $
% \begin{array}{rclr}
%             CoEM(v)& = & % \{
%            \displaystyle \sum_{(u, v) \in \mathsf{InEdges(v)}} \frac{w_{uv} \times CoEM(u)}{\sum_{(w,v) \in \mathsf{InEdges(v)}}w_{wv}}
%            &
%            \mbox{Co-Training EM}
% \end{array}
% $


\clearpage
\subsection{Example Fusions}
\label{sec:example-fusions}

We saw 
the fusion of the \irule{Radius} use-case in the paper, \autoref{fig:radius-fusion},
and
the fusion of the \irule{RDS} use-case in \autoref{sec:multiple-rounds}.
% 
In this subsection, 
we present the fusion of the \irule{DS} and \irule{DRR} use-cases.

% Desugaring and fusion the use-case $\DS$:

\ \\
\ \\

$$
\small
\begin{array}{clr}
\multicolumn{2}{l}{
\DS(s)
}
\\ = &
% \\ & =

\displaystyle
\bigcup_{
    v \in \Vertices \, \land \,
    \displaystyle
    \left(
    \min_{  p \in \Paths(s, v) } 
    \weight(p)
    \right)
    > 7
}
\{v\}
&
\mbox{By \irule{FMRed}}
\\ = &
% \\ & =

\displaystyle
% \bigcup_{
\underset{v \in \Vertices }{\R}
\ 
\left\<
    \displaystyle
    \left(
    \min_{  p \in \Paths(s, v) } 
    \weight(p)
    \right) > 7,
    \{v\}
\right\>
\mbox{\ \ where \ \ }
\begin{array}{l}
\R (b, \<a', b'\>) \coloneqq
\\ \t
    \lif \ (a') \lthen b \union b'
\\ \t
    \lelse \ b
%
% \\
% \R (\<a, b\>, \<a', b'\>) \coloneqq
% \\ \t
%     \lif \ (a \land a') \lthen b \union b'
% \\ \t
%     \lelse \ \lif \ (a) \lthen b
% \\ \t
%     \lese \ \lif \ (a') \lthen b'
% \\ \t
%     \lesel \ b
\end{array}
&
\mbox{By \irule{FPRed} and \irule{FILit}}
\\
\\ = &
% \\ & =



\displaystyle
% \bigcup_{
\underset{v \in \Vertices }{\R}
\ 
% \left
\<
    \displaystyle
    \left(
        \ilet x \coloneqq
        \underset{s}{\min} \ \weight
        \lin
        x
    \right) >
    \ilet x' \coloneqq \bot \lin 7,
\\ & \phantom{ \displaystyle \underset{v \in \Vertices }{\R} \ \< }
    \ilet x'' \coloneqq \bot \lin \{v\}
% \right
\>
\mbox{\ \ where \ \ }
\begin{array}{l}
\R (b, \<a', b'\>) \coloneqq
\\ \t
    \lif \ (a') \lthen b \union b'
\\ \t
    \lelse \ b
\end{array}
&
\mbox{By \irule{FILetBin}} 
\\ = &
% \\ & =



\displaystyle
\underset{v \in \Vertices }{\R}
\ 
\left(
\ilet \<\<x, x'\>, x''\> \coloneqq
    \<\<\underset{s}{\min} \ \weight, \bot\>, \bot\>
%     \displaystyle \min_{  p \in \Paths(s, v) } \weight(p) 
\lin
\left\<
    x > 7,
    \{v\}
\right\>
\right)
&
\mbox{By \irule{FMPairp}}
\\
\\ = &
% \\ & =



\displaystyle
\underset{v \in \Vertices }{\R}
\ 
\left(
\ilet x \coloneqq
    \underset{s}{\min} \ \weight
%     \displaystyle \min_{  p \in \Paths(s, v) } \weight(p) 
\lin
\left\<
    x > 7,
    \{v\}
\right\>
\right)
&
\mbox{By \irule{FVRed}}
\\
\\ = &


\left(
\begin{array}{l}
\ilet x \coloneqq 
%     \displaystyle \min_{  p \in \Paths(s, v) } \weight(p) 
    \underset{s}{\min} \ \weight
\lin
\\ 
\mlet x' \coloneqq 
    \left\<
        x > 7,
        \{v\}
    \right\>
\lin
\\ 
\rlet x'' \coloneqq 
%     \underset{v \in \Vertices}{\R'} \ x'
    \R \ x'
\lin
\\
x''
\end{array}
\right)
% 
\mbox{\ \ where \ \ }
\begin{array}{l}
\R (b, \<a', b'\>) \coloneqq
\\ \t
    \lif \ (a') \lthen b \union b'
\\ \t
    \lelse \ b
\end{array}


\end{array}
$$


% \ \\
% \ \\




$$
\small
\begin{array}{rclr}
    \DRR & = &
    \displaystyle
    \frac{
        \Diam
    }{
        \Radius
    }
    &
%     \mbox{Diameter to Radius Ratio}
    \\
    \\
    & = &
    \displaystyle
    \frac{
        \displaystyle \max_{s \in \{s_1, s_2\}} 
        \displaystyle \max_{v \in \Vertices} 
        \min_{ p \in \Paths(s,v)} \length(p)
    }{
        \displaystyle \min_{s \in \{s_1, s_2\}} 
        \displaystyle \max_{v \in \Vertices} 
        \min_{ p \in \Paths(s,v)} \length(p)
    }
    &
    \mbox{Similar to \autoref{fig:radius-fusion} for}
    \\
    &&&
    \mbox{\textsc{Radius} in the paper.}
    
    \\
    \\ 
    & = &
    \displaystyle
    \frac{
        \left(
        \begin{array}{l}
        \ilet \<x_1, y_1\> \coloneqq 
            \underset{\<s_1, s_2\>}{\min} \ \F
            \lin
        \\ 
        \mlet \<x_1', y_1'\> \coloneqq \<x_1, y_1\> \lin
        \\ 
        \rlet \<x_1'', y_1''\> \coloneqq 
            \R \ \< x_1',  y_1' \>
            \lin
        \\
        \max(x_1'', y_1'')
        \end{array}
        \right)
    }{
        \left(
        \begin{array}{l}
        \ilet \<x_2, y_2\> \coloneqq 
            \underset{\<s_1, s_2\>}{\min} \ \F
            \lin
        \\ 
        \mlet \<x_2', y_2'\> \coloneqq \<x_2, y_2\> \lin
        \\ 
        \rlet \<x_2'', y_2''\> \coloneqq 
            \R \ \< x_2',  y_2' \>
            \lin
        \\
        \min(x_2'', y_2'')
        \end{array}
        \right)
%         \mbox{\ \ where \ \ }
%         \begin{array}{l}
%         \F \coloneqq \lambda p. \ \left\< \length(p), \length(p) \right\> 
%         \\
%         \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
%         \\ \t
%         \<\max (a, a'), \max (b,  b') \>
%         \end{array}
    }
    \mbox{\ \ where \ \ }
    \begin{array}{l}
    \F \coloneqq \lambda p. \ \left\< \length(p), \length(p) \right\> 
    \\
    \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
    \\ \t
    \<\max (a, a'), \max (b,  b') \>
    \end{array}
    &
    \mbox{By \irule{FLetsBin}}

    
    \\
    \\
    & = &
    \displaystyle
        \left(
        \begin{array}{l}
        \ilet \<\<x_1, y_1\>, \<x_2, y_2\>\> \coloneqq 
            \<\underset{\<s_1, s_2\>}{\min} \ \F,
               \underset{\<s_1, s_2\>}{\min} \ \F\>
            \lin
        \\ 
        \mlet \<\<x_1', y_1'\>, \<x_2, y_2\>\> \coloneqq 
            \<\<x_1, y_1\>, \<x_2, y_2\>\>
            \lin
        \\ 
        \rlet \<\<x_1'', y_1''\>, \<x_2'', y_2''\>\> \coloneqq 
            \<\R \ \< x_1',  y_1' \>, 
               \R \ \< x_2',  y_2' \>\>
            \lin
        \\
        \max(x_1'', y_1'') / \min(x_2'', y_2'')
        \end{array}
        \right)
    &
    \begin{array}{r}
    \mbox{By \irule{IElim}}
    \\
    \mbox{Common}
    \\
    \mbox{path-based} 
    \\
    \mbox{reduction}
    \\
    \mbox{elimination}
    \end{array}
    \\ &&
%     \\ &&
%         \mbox{\ \ where \ \ }
%         \begin{array}{l}
%         \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
%         \\ \t
%         \<\max (a, a'), \max (b,  b') \>
%         \end{array}


    \\
    \\
    & = &
    \displaystyle
        \left(
        \begin{array}{l}
        \ilet \<x_1, y_1\> \coloneqq 
            \underset{\<s_1, s_2\>}{\min} \ \F
            \lin
        \\ 
        \mlet \<\<x_1', y_1'\>, \<x_2, y_2\>\> \coloneqq 
            \<\<x_1, y_1\>, \<x_1, y_1\>\>
            \lin
        \\ 
        \rlet \<\<x_1'', y_1''\>, \<x_2'', y_2''\>\> \coloneqq 
            \<\R \ \< x_1',  y_1' \>, 
               \R \ \< x_2',  y_2' \>\>
            \lin
        \\
        \max(x_1'', y_1'') / \min(x_2'', y_2'')
        \end{array}
        \right)
    &
    \begin{array}{r}
    \mbox{Similarly, }
    \\
    \mbox{by Common}
    \\
    \mbox{vertex-based} 
    \\
    \mbox{mapping}
    \\
    \mbox{elimination}
    \end{array}
    \\ &&
%     \\ &&
%         \mbox{\ \ where \ \ }
%         \begin{array}{l}
%         \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
%         \\ \t
%         \<\max (a, a'), \max (b,  b') \>
%         \end{array}


    \\
    \\
    & = &
    \displaystyle
        \left(
        \begin{array}{l}
        \ilet \<x_1, y_1\> \coloneqq 
            \underset{\<s_1, s_2\>}{\min} \ \F
            \lin
        \\ 
        \mlet \<x_1', y_1'\> \coloneqq 
            \<x_1, y_1\>
            \lin
        \\ 
        \rlet \<\<x_1'', y_1''\>, \<x_2'', y_2''\>\> \coloneqq 
            \<\R \ \< x_1',  y_1' \>, 
               \R \ \< x_1',  y_1' \>\>
            \lin
        \\
        \max(x_1'', y_1'') / \min(x_2'', y_2'')
        \end{array}
        \right)
    &
    \begin{array}{r}
    \mbox{Similarly, }
    \\
    \mbox{by Common}
    \\
    \mbox{vertex-based} 
    \\
    \mbox{reduction}
    \\
    \mbox{elimination}
    \end{array}
    \\ &&
%     \\ &&
%         \mbox{\ \ where \ \ }
%         \begin{array}{l}
%         \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
%         \\ \t
%         \<\max (a, a'), \max (b,  b') \>
%         \end{array}

        
    \\
    \\
    & = &
    \displaystyle
        \left(
        \begin{array}{l}
        \ilet \<x_1, y_1\> \coloneqq 
            \underset{\<s_1, s_2\>}{\min} \ \F
            \lin
        \\ 
        \mlet \<x_1', y_1'\> \coloneqq 
            \<x_1, y_1\>
            \lin
        \\ 
        \rlet \<x_1'', y_1''\> \coloneqq 
            \R \ \< x_1',  y_1' \>   
            \lin
        \\
        \max(x_1'', y_1'') / \min(x_1'', y_2'')
        \end{array}
        \right)
%     &
%     \begin{array}{r}
%     \mbox{Similarly, }
%     \\
%     \mbox{by Common}
%     \\
%     \mbox{vertex-based} 
%     \\
%     \mbox{reduction}
%     \\
%     \mbox{elimination}
%     \end{array}
%     \\ &&
%     \\ &&
        \mbox{\ \ where \ \ }
        \begin{array}{l}
        \F \coloneqq \lambda p. \ \left\< \length(p), \length(p) \right\> 
        \\
        \R \, ( \<a, b\>, \<a', b'\> ) \coloneqq
        \\ \t
        \<\max (a, a'), \max (b,  b') \>
        \end{array}
        
\end{array}
$$















==> SynthesisApp.tex <==
\clearpage
\section{Mapping Specification to Iteration-Map-Reduce}
\subsection{Iterative Reduction and its Correctness}
\label{sec:iter-red-app}
We consider four variants of iterative reduction based on
whether the values of the predecessors are 
pulled by the vertex itself or
pushed by the predecessors,
and
whether the reduction function $\R$ is idempotent.
\subsubsection{Pull Model }
\label{sec:pull-iter-correctness}
% \hfill\\
\ \

% The pull model is completely presented in the main body \autoref{sec:iter-reduction}.





\textit{Pull model with idempotent reduction. \ }
% \subsubsubsection{Pull model with idempotent reduction. \ }

\begin{theorem}[Correctness of Pull (idempotent reduction)]
\label{thm:iteration-pull-app-text}
For all $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
% if the conditions $\CB_1$ - $\CB_5$ and $\CB_7$ - $\CB_{10}$ hold,
if the conditions $\CB_1$ - $\CB_{9}$ hold,
then
$
\S_\pulli^k(v) = 
\Spec^k(v)
$.
\end{theorem}


The full proof is available in 
the appendix \autoref{sec:proofs-pull-i}.
% \appref{\secProofsPullI}.
We prove by induction that after each iteration $k$,
the value $\S_\pulli^k(v)$ of each vertex $v$ 
is $\Spec^k(v)$ that is the reduction over paths to $v$ of length less than $k$.
% 
% The proof is by induction.
At the iteration $k=1$,
% beginning with 
% there is only a path of length zero from the source(s) to itself.
the specification $\Spec^1(v)$
requires
reduction on 
only the paths of length zero to each vertex.
% should be considered.
% 
Therefore,
by the conditions $\CB_1$ - $\CB_2$,
the initialization function $\I$ properly
initializes 
% the value of only the source vertex (or vertices).
each vertex $v$ to $\Spec^1(v)$.
% 
In each iteration $k+1$,
if there is any predecessor of the vertex $v$
whose value is changed
in the previous iteration $k$,
then 
their new values are propagated by $\P$
and reduced together by $\R$
and then reduced with the current value of $v$.
By the conditions $\CB_7$ and $\CB_8$, the reduction function $\R$ is commutative and associative, and can be applied to the propagated values in any order.
By the induction hypothesis, the value of each predecessor $u$
is the reduction of the paths to $u$ of length $l$, $0 \leq l < k$.
% less than $k$.
The predecessors that have no paths and store $\bot$ are ignored by the conditions $\CB_3$ and $\CB_7$.
By the conditions $\CB_3$, $\CB_4$ and $\CB_5$,
the propagation of the value of a predecessor $u$ of the vertex $v$
% results in 
is equal to
the reduction over the paths to $v$ that pass through $u$.
Since these paths include at least the edge (from $u$ to $v$),
their length $l$ is $0 < l < k+1$.
% greater than zero and less than $k+1$.
The previous value of $v$ itself is
the reduction over paths to $v$ of 
% length less than $k$.
length $l$, $0 \leq l < k$.
Since, the reduction function $\R$ is idempotent,
reducing these two values
absorbs the values of the repeated paths and
results in the reduction over all paths of length $l$, $0 \leq l < k+1$.
% less than $k+1$ (including length zero).
If the value of none of the predecessors is changed in the previous iteration,
% $k-1$,
then the above reduction is skipped,
% but then 
and
it can be shown that the current value of the vertex is already equal to the above reduction.
% of values.


\clearpage
\textit{Pull model with non-idempotent reduction. \ }


% \mclearpage
% \noindent
\begin{theorem}[Correctness of Pull (non-idempotent reduction)]
\label{thm:iteration-pull-noni-app-text}
% \ \\ \t
For all $\R$, $\F$, 
% $\C$, 
$\I$, $\P$, $k \geq 1$, and $s$,
% \ \\ \t
let $\C(p) \coloneqq (\head(p) = s)$,
% \ \\ \t
% if the conditions $\CB_1$ - $\CB_5$ and $\CB_7$ - $\CB_9$ hold, 
if the conditions $\CB_1$ - $\CB_8$ hold, 
and
$s$ is not on any cycle,
% \ \\ \t
$
\S_\pulln^k(v) = 
\Spec^k(v)
% \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$.
\end{theorem}




The full proof is available in 
the appendix \autoref{sec:proofs-pull-n}.
% \appref{\secProofsPullN}.
The proof of this theorem
is similar to the proof of
% \autoref{thm:iteration-pull-app-text}.
\autoref{thm:iteration-pull-app-text}.
% the main difference is
% avoiding reduction with the previous value of the vertex.
% 
% The main difference is that 
% the current value of the vertex $v$ is not reduced with 
% the propagated values from the predecessors
% to avoid redundant paths.
Based on the induction hypothesis,
% in iteration $k$,
% the reduction of the values propagated from the predecessors
the reduction of the propagated values
covers the paths of length $l$, $0 < l < k + 1$.
The current value of $v$ itself covers the paths of length $l$, $0 \leq l < k$.
% The intersection is the paths of length $l$, $0 < l < k$.
Since the two sets of paths overlap 
and the reduction function may not be idempotent,
the reduction with the latter is avoided.
However, no path is missed by avoiding the reduction.
The difference is only the paths of length $0$.
The vertices other than the source $s$ do not have a path of length $0$ from $s$.
The source $s$ is correctly initialized to the value of $\F$ on the zero-length path $\<s, s\>$ from $s$ to itself,
and 
since $s$ is not on any cycle,
% stays unchanged 
% its value is never updated; it keeps its correct value.
% it never overwrites its correct value.
its correct value is never overwritten.
% and keeps its correct value.

\clearpage
\subsubsection{Push Model}
\label{sec:push-iter-correctness}
\ \



% The push model was presented in the main body \autoref{sec:iter-reduction}.
% We present the the elided proof intuitions in this subsection



\textit{Push model with idempotent reduction. \ }
 



% \noindent
\begin{theorem}[Correctness of Push (idempotent reduction)]
\label{thm:iteration-push-app-text}
% \ \\ \t
For all $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
% if the conditions $\CB_1$ - $\CB_5$ and $\CB_7$ - $\CB_{10}$ hold,
if the conditions $\CB_1$ - $\CB_9$ hold,
% \ \\ \t
$
\S_\pushi^k(v) = 
\Spec^k(v)
% \undersetp{
% %     \{ p \ | \ \exists v'. \ \path(p, v', v) \; \land \; \C(p) \; \land \; \length(p) \leq k \} 
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$.
\end{theorem}


The full proof is available in \autoref{sec:proofs-push-i}.
% the appendix \autoref{sec:proofs-push-i}.
%\appref{\secProofsPushI}.
% The proof 
% % of this theorem 
% is similar to the proof of \autoref{thm:iteration-pull}.
% 
Similar to the proof of \autoref{thm:iteration-pull-app-text},
the reduction function should be idempotent since
the reduced values may cover overlapping sets of paths.
% 
The main difference is that
% to calculate the value of the vertex $v$ at iteration $k$,
instead of propagating and reducing the values of all the predecessors of $v$,
only the values of the predecessors $\{ \overline{u} \}$ 
of $v$ 
that have been changed in the previous iteration $k$ 
are propagated and reduced.
% push their values and reduce them with the current value of $v$.
% The main difference is that
% to calculate the value of the vertex $v$ at iteration $k$,
% instead of pulling and reducing the values of all the predecessors,
% only the predecessors $\{ \overline{u} \}$ of $v$ that have changed values in the previous iteration $k-1$
% push their values and reduce them with the current value of $v$.
% 
Therefore, the values of the unchanged predecessors $\{ \overline{w} \}$ of $v$
% are not pushed and 
are not reduced with the current value of $v$.
However, 
% the reduced value stored at $v$
the resulting value of $v$
does not miss 
any path to $v$ that goes through an unchanged predecessor $w$.
If $w$ is never changed,
there is no path from the source(s) to it.
% 
If it is changed in the previous iterations,
in the last such iteration,
its value has been already reduced with the current value of $v$.



\clearpage
\textit{Push model with non-idempotent reduction. \ }
 

This model works
for non-idempotent (in addition to idempotent) reduction functions.
We consider two instances of this model:
first the basic and then the optimized iteration model.


The first variant of push, non-idempotent was defined in 
\autoref{fig:pull-push-iter},
\autoref{def:computation-push-noni}.

\noindent
\begin{theorem}[Correctness of Push (non-idempotent reduction) I]
\label{thm:iteration-push-noni-app-text}
\ \\ \t
For all $\R$, $\F$, 
% $\C$, 
$\I$, $\P$, $k \geq 1$, and $s$,
% \ \\ \t
let $\C(p) \coloneqq (\head(p) = s)$,
% \ \\ \t
if the conditions $\CB_1$ - $\CB_8$ hold, 
and
$s$ is not on any cycle,
% \ \\ \t
$
\S_\pushn^k(v) = 
\Spec^k(v)
$
\end{theorem}


The full proof is available in 
the appendix \autoref{sec:proofs-push-n}.
The proof of this theorem
is similar to the proof of
\autoref{thm:iteration-pull-noni-app-text}.
Based on the induction hypothesis,
the reduction of the propagated values
covers the paths of length $l$, $0 < l < k + 1$.
% The current value of $v$ itself covers the paths of length $l$, $0 \leq l < k$.
% Since the two sets of paths overlap 
% and the reduction function may not be idempotent,
% the reduction with the latter is avoided.
% No path is missed by avoiding the reduction.
Let us consider the paths of length $0$.
The vertices other than the source $s$ do not have a path of length $0$ from $s$.
The source $s$ is correctly initialized to the value of $\F$ on the zero-length path $\<s, s\>$ from $s$ to itself,
and 
since $s$ is not on any cycle,
its correct value is never overwritten.




\clearpage
The second variant 
% optimized iteration model
is represented in
% \autoref{fig:pull-push-iter},
% \autoref{def:computation-push-noni}.
\autoref{def:computation-push-noni-opt-text} below.
% 
Let the value of the vertex $v$ in the iteration $k$ be represented as $\S_\pushn^k(v)$.
% 
%The push model for non-idempotent reduction 
% 
The main difference with 
% the push model for idempotent reduction
the previous model
is that 
every changed predecessor $u_i$ first rollbacks its previous update before applying its new update.
% 
The rollback function $\B$, given a value $n$ and an edge $\<u,v\>$
where $n$ is the previous value of $u$,
defines the value that is propagated to $v$ to be rolled back.
% The rollback function $\B$, given a value $n$ and an edge $e$
% where $n$ is the previous value of the source of $e$,
% defines the value that is propagated to the destination of $e$ to be rolled back.
The rollback value is expected to cancel the previously propagated value.
For example, for the \textsc{PageRank} use-case as \autoref{fig:iter-kern-exam} shows,
the rollback function returns the negation of the previously propagated value.
%
For each predecessor $u_i$,
the rollback function $\B$ is applied to 
% the previously propagated value 
the previous value 
$\S_\pushn^{k-1}(u_i)$ of $u_i$
and the edge $\<u_i, v\>$,
and 
the propagate function $\P$ is applied to
the latest value $\S_\pushn^{k}(u_i)$ of $u_i$
and the edge $\<u_i, v\>$.
The two resulting values are reduced with the current value of $v$.



 
% \noindent
\begin{definition}[Push (non-idempotent reduction) II]
% \label{def:comp-push}
\label{def:computation-push-noni-opt-text}
% \ \\ \t
$$
\begin{array}{ll}
\S_\pushn^0(v) \coloneqq \bot
\ \\
\S_\pushn^1(v) \coloneqq \I(v)
\ \\
\S_\pushn^{k+1}(v) \coloneqq 
\E(S_n),
\ \ \ 
k \geq 1
\mbox{\ \ \ where \ }
\ \\ \t
\llet \{u_{0}, .., u_{n-1} \} \coloneqq
\CPreds^k(v) \lin
% \left\{ u \ | \ u \in \preds(v) \land \S_\pushi^k(u) \neq \S_\pushi^{k-1}(u) \right\}
\ \\ \t
S_0 \coloneqq \S_\pushn^{k}(v)
\ \\ \t
S_{i+1} \coloneqq \R ( \R( S_{i},
% \left( 
\ \\ \t\t
\ \B \left( \S_\pushn^{k-1}(u_i), \<u_i, v\> \right)),
\ \\ \t\t
\ \P \! \left( \S_\pushn^k(u_i), \<u_i, v\> \right)
% \right)
)
\end{array}
$$
\end{definition}



% \begin{definition}[Page-rank specification]
% % \label{def:comp-push}
% \label{def:page-rank-spec}
% $$
% \begin{array}{rclr}
%     \multicolumn{3}{l}{\textsc{PageRank}} 
%     \\
%     \ \ \ \ 
%     \I & \coloneqq &
%         \lambda v. \ \ 
%         1 \, / \, |V|
%     \\
%     \P & \coloneqq &
%         \lambda n, e. \ \ 
%         n \, / \, \mathsf{outdeg}(\mathsf{src}(e))
%     \\
%     \R & \coloneqq &
% %         +
%         \lambda v, v'. \ \ 
%         v + v'
%     \\
%     \E & \coloneqq &
%         \lambda n. \ \ 
%         \gamma * n \,\, + \,\, (1-\gamma) \, / \, |V|
%     \\
%     \B & \coloneqq &
%         \lambda n, e. \ \ 
%         -n \, / \, \mathsf{outdeg}(\mathsf{src}(e))
% \end{array}
% % \\
% \\
% \multicolumn{1}{c}{\mbox{(b) Examples}}
% \end{array}
% $$
% \end{definition} 


The correctness of this variant of iteration is dependent on the following condition for the propagation and rollback functions.

$$
\begin{array}{l}
\CB_{11} \ (\mbox{Rollback})\colon 
\\ \t\t
\forall n, n'. \ 
% \\ \t\t\t
\R ( n, \R (
%     \R(
%         \F(p_1 \cdot \<u, v\>),
%         \F(p_2 \cdot \<u, v\>)
%     ), \
%     n
%     \P(n', \<u, v\>),
    \P(n', e),
\\ \t\t \phantom{\forall n, n'. \ \R ( n \R (} \ 
    \B\left(
%         \R(\F(p_1), \F(p_2)), \
        n', 
%         \<u, v\>
        e
    \right))) = n
\end{array}
$$


As we saw in 
% \autoref{fig:pull-push-iter},
\autoref{def:computation-push-noni-opt-text},
in this variant of push model with non-idempotent reduction
$\S_\pushn^k(v)$,
each predecessor first rollbacks its previously propagated value before propagating its new value.
The rollback value is expected to cancel the previously propagated value.
% 
This requirement is captured as the condition $\CB_{11}$ above.
% in \autoref{fig:correct-conds}.
% 
As an example,
%consider the factored path-based reduction 
%$\underset{s}{\sum} \, 1$ 
%that counts the number of paths from the source $s$.
%The propagate function $\P = \lambda n, e. \ n$ returns the value of the predecessor,
%and
%the rollback function $\B = \lambda n, e. \ {-n}$ returns the negation of the previous value of the predecessor.
% 
% 
%As another example,
the number of shortest paths use-case \irule{NSP},
after fusion, 
calculates a pair for each vertex where 
the first element is the shortest path weight 
and 
the second element is the number of such paths.
% 
For \irule{NSP},
the propagate function is $\P = \lambda \<w, n\>, e. \ \<w, n\>$
and
the rollback function is $\B = \lambda \<w, n\>, e. \ \<w, {-n}\>$.


% For the push model with non-idempotent reduction,
For synthesis in this model,
after the propagation function $\P$ is synthesized,
the condition $\CB_{11}$ is used to synthesize the rollback function $\B$.

  
The following theorem states that 
if the conditions $\CB_1$ - $\CB_8$ 
% (in particular the condition $\CB_6$)
and the condition $\CB_{11}$
hold,
% if the condition $\CB_6$ in addition to 
% the same conditions as for the previous model
% the pull model 
% idempotent model
% for the idempotent model 
% except idempotency
% hold,
this model
% (\autoref{def:computation-push-noni})
% the push model for non-idempotent reduction $\S_\pushn^k(v)$ 
complies with
% of each vertex $v$ is 
the specification $\Spec^k(v)$.



% % \noindent
% \begin{theorem}[Correctness of push (non-idempotent reduction)]
% \label{thm:iteration-push-noni}
% % \ \\ \t
% For all $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
% if the conditions $\CB_1$ - $\CB_9$ hold,
% % \ \\ \t
% $
% \S_\pushn^k(v) = 
% \Spec^k(v)
% % \undersetp{
% %     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% % }{\R} \ \F(p)
% $.
% \end{theorem}


\begin{theorem}[Correctness of Push (non-idempotent reduction) II]
\label{thm:iteration-push-noni-app}
% \ \\ \t
For all $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
if the conditions $\CB_1$ - $\CB_8$ and $\CB_{11}$ hold,
% \ \\ \t
$
\S_\pushn^k(v) = 
\Spec^k(v)
% \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$.
\end{theorem}


The full proof is available in \autoref{sec:proofs-push-n}.
% the appendix \autoref{sec:proofs-push-n}.
%\appref{\secProofsPushN}.
First, we show that after each iteration $k+1$,
the value of each vertex $v$ is 
the reduction of its initial value and
the value of predecessors in the previous iteration $k$.
%
Even though only the changed predecessors push values,
similar to the proof of \autoref{thm:iteration-push-app-text},
the value of no predecessor is missed.
% 
If a predecessor is never changed,
it has the value $\bot$ that is ignored in the reduction anyway.
If it is changed in the previous iterations,
in the last such iteration,
its value has been 
% pushed to
pushed and reduced with
% reduced with 
the current value of $v$.
Since reduction is not idempotent,
each predecessor first rollbacks its old value 
before applying its new value.
% 
Second,
using the first fact,
we show by induction that 
% the result of reduction
the value of each vertex $v$
is the reduction of the paths to $v$ of length less than $k+1$.
% 
Similar to the previous proofs,
it can be shown that
the initial value of $v$ is 
the result of reduction on paths to $v$ of length $0$.
% 
Further, using the induction hypothesis, it can be shown that 
the propagation of values from the predecessors in iteration $k+1$
results in
% is equal to 
the reduction over paths to $v$ of length $l$, $0< l < k+1$.
% 
Reducing the two values results in
the reduction over paths to $v$ of length $l$, $0 \leq l < k+1$ 
% (including $0$)
that the specification $\Spec^{k+1}(v)$ requires.



\clearpage

\subsubsection{Asynchronous Model}
\ \ \

\label{sec:asynchronous}

% \begin{figure*}[h!]
\begin{figure}[h!]
% \begin{figure*}[t!]
\small

$
\begin{array}{l}
\mbox{The predecessors of the vertex $v$ that changed value in the iteration $k$:}
\\
\CPreds^k(v) = 
\left\{ u \ | \ u \in \preds(v) \land \S^k(u) \neq \S^{k-1}(u) \right\}
\end{array}
$

% \noindent
\begin{definition}[Pull (idempotent reduction)]
\label{def:a-computation-pull}
% \ \\ \t
$$
\begin{array}{ll}
\S_\apulli^0(v) \coloneqq \bot
\ \\
\S_\apulli^1(v) \coloneqq \I(v)
\ \\
\S_\apulli^{k+1}(v) \coloneqq
\twopartdef{
    \S_\apulli^k(v)
}{
    \CPreds^k(v) = \emptyset
}{
    \E \left[
    \R \left(
        \S_\apulli^k(v), \ 
        \undersetp{ \, u \in \preds(v) }{\R}
%         \left( 
        \, \P \! \left( \S_\apulli^k(u) \, ? \, \S_\apulli^{k+1}(u), \<u, v\> \right)
%         \right)
    \right)
    \right]
}
k \geq 1
&
%     k \geq 1
\end{array}
$$
\end{definition}


% \noindent
\begin{definition}[Pull (non-idempotent reduction)]
\label{def:a-computation-pull-noni}
% \ \\ \t
$$
\begin{array}{ll}
\S_\apulln^0(v) \coloneqq \bot
\ \\
\S_\apulln^1(v) \coloneqq \I(v)
\ \\
\S_\apulln^{k+1}(v) \coloneqq
\twopartdef{
    \S_\apulln^k(v)
}{
    \CPreds^k(v) = \emptyset
}{
    \E \left[
        \undersetp{ \, u \in \preds(v) }{\R}
        \, \P \! \left( \S_\apulln^k(u) \, ? \, \S_\apulln^{k+1}(u), \<u, v\> \right)
    \right]
}
&
    k \geq 1
\end{array}
$$
\end{definition}



% \begin{tabular}{ll}

% \begin{minipage}{\textwidth/2}

% \noindent
\begin{definition}[Push (idempotent reduction)]
% \label{def:comp-push}
\label{def:a-computation-push}
% \ \\ \t
$$
\begin{array}{ll}
\S_\apushi^0(v) \coloneqq \bot
\ \\
\S_\apushi^1(v) \coloneqq \I(v)
% \ \\
% \S_\apushi^{1}(v) \coloneqq
%     \R \left[  
%         \undersetp{\{ u \ | \ u \in \preds(v) \; \land \; \S_\apushi^0(u) \neq \bot \} }{\R} 
%             \left[ \P (\S_\apushi^0(u), \<u, v\>)
%     \right] \!, \ 
%     \S_\apushi^{0}(v)
%     \right]
\ \\
\S_\apushi^{k+1}(v) \coloneqq \E(S_n),
\ \ \ 
k \geq 1
\mbox{\ \ \ where \ }
\ \\ \t
\llet \{u_0, .., u_{n-1} \} \coloneqq
\CPreds^k(v) \lin
\ \\ \t
\llet m_i \coloneqq
|\CPreds^k(u_i)| \lin
% \left\{ u \ | \ u \in \preds(v) \land \S_\apushi^k(u) \neq \S_\apushi^{k-1}(u) \right\}
\ \\ \t
S_0(v) \coloneqq \S_\apushi^{k}(v)
\ \\ \t
S_{i+1}(v) \coloneqq \R \left( S_{i}(v), \ 
    \P \! \left( ?_{j\in\{1..m_i\}} \, S_{j}(u_i), \<u_i, v\> \right) 
\right)
\end{array}
$$
\end{definition}

% \end{minipage}

% &

% \begin{minipage}{\textwidth/2}

% \noindent
\begin{definition}[Push (non-idempotent reduction)]
% \label{def:comp-push}
\label{def:a-computation-push-noni}
% \ \\ \t
$$
\begin{array}{ll}
\S_\apushn^0(v) \coloneqq \bot
\ \\
\S_\apushn^1(v) \coloneqq \I(v)
\ \\
\S_\apushn^{k+1}(v) \coloneqq \E(S_n(v)),
\ \ \ 
k \geq 1
\mbox{\ \ \ where \ }
\ \\ \t
\llet \{u_0, .., u_{n-1} \} \coloneqq
\CPreds^k(v) \lin
% \left\{ u \ | \ u \in \preds(v) \land \S_\apushi^k(u) \neq \S_\apushi^{k-1}(u) \right\}
% \ \\ \t
% \llet m_i \coloneqq
% |\CPreds^k(u_i)| \lin\
\\ \t
S_0(v) \coloneqq
\S_\apushn^{k}(v)
\ \\ \t
S_{i+1}(v) \coloneqq 
\R ( \R( S_{i}(v),
% \left( 
\ \\ \t\t
\ \B \left( 
% \S_\pushn^{k-1}(u_i), 
% ?_{j\in\{1..m_i\}} \, S_{j}(u_i),
b^{k-1}(u_i),
\<u_i, v\> \right)),
\ \\ \t\t
\ \P \! \left( 
% \S_\pushn^k(u_i), 
b^k(u_i), 
\<u_i, v\> 
\right))
% 
% \R \left( 
%     S_{i}(v), \ 
%     \P \! \left( ?_{j\in\{1..m_i\}} \, S_{j}(u_i), \<u_i, v\> \right) 
% \right)
% 
\ \\ \t
b^{k+1}(v) \coloneqq \ ?_{i \in \{0..n\}} \, S_{i}(v)

% \ \\
% \S_\apushn^{k+1}(v) \coloneqq 
% S_{n}(v)

% \R ( \R( S_{i},
% % \left( 
% \ \\ \t\t
% \ \B \left( 
% \S_\pushn^{k-1}(u_i), 
% \<u_i, v\> \right))
% \ \\ \t\t
% \ \P \! \left( \S_\pushn^k(u_i), \<u_i, v\> \right))

% % \left( 
% \ \\ \t\t
% \ \B \left( \S_\apushn^{k-1}(u_i), \<u_i, v\> \right))
% \ \\ \t\t
% \ \P \! \left( \S_\apushn^k(u_i), \<u_i, v\> \right)
% % \right)
% )
\end{array}
$$
\end{definition}

% \end{minipage}
% \end{tabular}

\caption{
    Four Iterative Reduction Methods (in the asynchronous mode). The operator $?$ is the non-deterministic choice operator.
}
\label{fig:a-pull-push-iter}
% \end{figure*}
\end{figure}



The iteration models that were presented in \autoref{fig:pull-push-iter} are \emph{synchronous}.
In the synchronous model, 
in each iteration $k+1$,
each vertex $v$ stores both its previous value $\S^k(v)$
and its new value $\S^{k+1}(v)$.
% 
The previous value $\S^k(v)$ of $v$ is propagated to update other vertices
and
updates to the value of $v$ are stored in its new value $\S^{k+1}(v)$.
%
Therefore, the updates in the current iteration do not affect the values that are propagated.
%
In the \emph{asynchronous} model, however, each vertex stores one value.
The single value is used to both propagate the current value of the vertex
and store its new value.
Asynchronous model can save space and converge faster
but is more subtle.
% makes reasoning about correctness more complicated.
The values that are propagated in iteration $k+1$
can be either 
the previous value
$\S^{k}(v)$,
the old value
$\S^{k+1}(v)$
% of $v$
or
an intermediate value between the two.
% 
The high-level idea 
% for the correctness 
is that
the new value has more information than the old value
i.e.\ covers more paths.
Thus, vertices reach 
% the final values faster.
% the convergent values 
convergence
faster.
% where 
% additional paths do not change.
% that should be eventually considered.
% $\S^{k+1}(v)$





The asynchronous pull model for idempotent and non-idempotent reduction functions are presented in
\autoref{def:a-computation-pull} and \autoref{def:a-computation-pull-noni}.
They are very similar to the corresponding synchronous pull models that were presented in
\autoref{def:computation-pull} and \autoref{def:computation-pull-noni}.
Now, the propagated value is either the previous value
$\S_\apulli^k(u)$
or the new value
$\S_\apulli^{k+1}(u)$
of the predecessor $u$.
The operator $?$ is the non-deterministic choice operator that non-deterministically returns one if its operands.



The asynchronous push model for idempotent reduction functions is presented in
\autoref{def:a-computation-push}.
It is similar to the corresponding synchronous definition presented in
\autoref{def:computation-push}.
The difference is that 
instead of the previous value $\S_\pushi^k(u_i)$ of each predecessor $u_i$,
one of its intermediate values $S_{j}(u_i)$ is propagated.
Assuming that the predecessor $u_i$ has $m_i$ changed predecessors itself,
$u_i$ has the intermediate values $S_{j}(u)$ where ${j\in\{1..m_i\}}$,
one after each push from its predecessors.
% 
The value propagated to $v$ can non-deterministically be any of the intermediate values.




The asynchronous push model for non-idempotent reduction functions is presented in
\autoref{def:a-computation-push-noni}.
% In contrast to the previous definitions, it is not similar to the corresponding synchronous definition presented in \autoref{def:computation-push-noni}.
It not similar to the corresponding synchronous definition presented in \autoref{def:computation-push-noni}.
% In fact, it is more similar to the pull model for non-idempotent reduction functions
% presented in \autoref{def:computation-pull-noni}.
% The reason is that following the approach of the synchronous push model for non-idempotent reduction functions 
% presented in \autoref{def:computation-push-noni}
% would need to store the previously propagated value to roll it back before propagating the new value.
The difference is that 
the values propagated by a vertex can be any of its intermediate values and not necessarily its value at the end of the last iteration.
Thus, we need to store the previously propagated values to roll them back before propagating new values.
%
Consider a vertex $v$ and its predecessor $u_i$.
The value that $u_i$ propagates to $v$ in iteration $k$ is stored as $b^{k}(u_i)$.
In iteration $k+1$,
to push from the predecessor $u_i$ to the vertex $v$,
the value $b^{k-1}(u_i)$ is rolled back by the rollback function $\B$
and 
the new value $b^{k}(u_i)$ is propagated by the propagation function $\P$.
% In the synchronous model,
% the previously propagated value is 
% the value 
% $\S_\pushn^{k-1}(u_i)$
% available at vertex $u_i$ 
% when it is being updated to 
% the value $\S_\pushn^{k}(u_i)$
% that is propagated.
% However, in the asynchronous model
% the previously propagated value can be an intermediate value 
% that may not be overwritten later in the iteration
% and hence should be stored.
% Storing the previously propagated value defeats the goal of avoiding duplicate storage.
% Therefore, 
% the asynchronous push model for non-idempotent reduction functions, presented in
% \autoref{def:a-computation-push-noni},
% avoids keeping track of the previously propagated values and rollbacks.
% Instead of rolling back the previous values,
% it recalculates the value of the vertex.
% Thus,
% in each iteration, 
% all vertices start from the none value $\bot$
% and
% instead of only the changed predecessors,
% all the predecessors push their (potentially intermediate) values.



We define
$P^\infty(v)$
as all the paths to the vertex $v$ (that satisfy the condition $\C$).

\begin{definition}[Paths]
% \begin{equation}
\label{def:a-full-paths}
% \begin{array}{l}
$
P^\infty(v) = \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \}
$
% \end{array}
% \end{equation}
\end{definition}

The definition of specification $\Spec(v)$ is the same as 
definition \autoref{def:red-spec}; only the paths are factored to $P^\infty(v)$.
% \autoref{def:a-full-red-spec}

\begin{definition}[Specification]
% \begin{equation}
\label{def:a-full-red-spec}
% \begin{array}{l}
$
\Spec(v) = 
% \displaystyle
% \underset{p \in \Paths(v) \; \land \; \C(p)}{\R} \F(p)
% \R_{ p \in \{p \, | \, p \in \Paths(v) \; \land \; \C(p) \} } \ \F(p)
\R_{ p \in P^\infty(v) } \ \F(p)
$
% \end{array}
% \end{equation}
\end{definition}

We define
$P^k(v)$
as the paths to the vertex $v$ of length less than $k$ (that satisfy the condition $\C$).

\begin{definition}[$k$-Paths]
% \begin{equation}
\label{def:a-full-k-paths}
% \begin{array}{l}
$
P^k(v) = \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
$
% \end{array}
% \end{equation}
\end{definition}

The definition of specification for iteration $k$, $\Spec^k(v)$, is the same as 
definition \autoref{def:red-spec-k}; only the paths are factored to $P^k(v)$.
% \autoref{def:a-full-red-spec}


\begin{definition}[$k$-Specification]
% [Specification of iteration $k$]
% \begin{equation}
\label{def:red-spec-k-app}
% \begin{equation}
$
\Spec^k(v)
=
\undersetp{
    p \, \in \, P^k(v)
}{\R} \ \F(p)
$
% \end{equation}
\end{definition}

Since in the asynchronous model, 
in an iteration $k$,
the value of vertices may cover paths of length $k$ or longer,
we define $aP^k(v)$
as the set of
paths that include paths of length less than $k$
and maybe more.


\begin{definition}[a-$k$-Paths]
% \begin{equation}
\label{def:a-k-paths}
% \begin{array}{l}
$
aP^k(v) = \{ P \, | \, P(k) \subseteq  P \subseteq P^\infty(v) \}
$
% \end{array}
% \end{equation}
\end{definition}


Since in the asynchronous model,
vertices may propagate any one of the multiple intermediate values,
we define asynchronous specification for iteration $k$, $\aSpec^k(v)$,
as set of values:
the reductions of any set of paths $P$ in $aP^k(v)$.


\begin{definition}[a-$k$-Specification]
% \begin{equation}
\label{def:a-red-spec-k}
% \begin{array}{l}
$
\aSpec^k(v)
=
\{
\undersetp{
    p \, \in \, P
}{\R} \ \F(p)
\, | \,
P \in aP^k(v)
\}
$
% \end{array}
% \end{equation}
\end{definition}


All the asynchronous models presented in
\autoref{fig:a-pull-push-iter}
comply with the asynchronous specification.
In each iteration,
the value stored at vertex $v$ is in the set of values
$\aSpec^k(v)$.


\begin{theorem}[Correctness of Pull (idempotent reduction)]
\label{thm:a-iteration-pull-app}
Forall $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_9$ hold,
then
$
\S_\apulli^k(v) \in
\aSpec^k(v)
$
\end{theorem}


The proof is similar to the proof of
\autoref{thm:iteration-pull-app-text}.
The set of paths covered by
$\S_\apulli^{k+1}(u)$
is a superset of path covered by
$\S_\apulli^k(u)$.
The reduction over the set of paths in the difference is factored out in the proof.


% \mclearpage
% \noindent
\begin{theorem}[Correctness of Pull (non-idempotent reduction)]
\label{thm:a-iteration-pull-noni-app}
% \ \\ \t
Forall $\R$, $\F$, 
% $\C$, 
$\I$, $\P$, $k \geq 1$, and $s$,
% \ \\ \t
let $\C(p) \coloneqq (\head(p) = s)$,
% \ \\ \t
if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_8$ hold, 
and
$s$ is not on any cycle,
% \ \\ \t
$
\S_\apulln^k(v) \in
\aSpec^k(v)
% \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$
\end{theorem}


The proof is similar to the proof of
\autoref{thm:iteration-pull-noni-app-text}.
The set of paths covered by
$\S_\apulli^{k+1}(u)$
is a superset of path covered by
$\S_\apulli^k(u)$.
The reduction over the set of paths in the difference is factored out in the proof.



% \noindent
\begin{theorem}[Correctness of Push (idempotent reduction)]
\label{thm:a-iteration-push-app}
% \ \\ \t
Forall $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_9$ hold,
% \ \\ \t
$
\S_\apushi^k(v) \in
\aSpec^k(v)
% \undersetp{
% %     \{ p \ | \ \exists v'. \ \path(p, v', v) \; \land \; \C(p) \; \land \; \length(p) \leq k \} 
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$
\end{theorem}


The proof is similar to the proof of
\autoref{thm:iteration-push-app-text}.
The set of paths covered by
$S_{j}(u_i)$
is a superset of path covered by
$\S_\pushi^k(u_i)$.
The reduction over the set of paths in the difference is factored out in the proof.




% \noindent
\begin{theorem}[Correctness of Push (non-idempotent reduction)]
\label{thm:a-iteration-push-noni-app}
% \ \\ \t
Forall $\R$, $\F$, $\C$, $\I$, $\P$, and $k \geq 1$,
if the conditions $\CB_1$ - $\CB_8$ hold,
% \ \\ \t
$
\S_\apushn^k(v) \in
\aSpec^k(v)
% \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
$
\end{theorem}


The proof is similar to the proof of
\autoref{thm:iteration-push-noni-app}.
% 
The set of paths covered by
$b_{k}(u_i)$
is a superset of path covered by
$\S_\pulln^k(u_i)$.
The reduction over the set of paths in the difference is factored out in the proof.



\begin{theorem}[Termination]
\label{thm:a-iteration-termination-app}
% \ \\ \t
Forall $\R$, $\F$, and $\C$, 
% let
% \ \\ \t
% $\Spec(v) = \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \}
% }{\R} \ \F(p)$ and
% \ \\ \t
% $
% \S^k(v) = \undersetp{
%     p \, \in \, \{ p \, | \, p \in \Paths(v) \; \land \; \C(p) \; \land \; \length(p) < k \}
% }{\R} \ \F(p)
% $.
% \ \\ \t
if 
the graph is acyclic or
the condition $\CB_{10}$ holds, then
there exists $k'$ such that for every $k \geq k'$,
% \ \\ \t
$\aSpec^{k}(v) = \{ \Spec(v) \}$.
% there exists $k$ such that
% % \ \\ \t
% $\Spec^{k}(v) = \Spec^{k +1}(v) = \Spec(v)$.
\end{theorem}


The proof is similar to the proof of 
\autoref{thm:iteration-termination-app}.
Let $l$ be 
% The paths longer than 
the longest simple path to $v$.
% do not change the result of the reduction.
If the graph is acyclic,
there is no path longer than $l$.
Thus, for any $k > l+1$, 
$P^k(v) = \{P^\infty(v)\}$.
Therefore, 
$\aSpec^{k}(v) = \{ \Spec(v) \}$.
% 
Even if the graph is cyclic,
% for any $P \in P^k(v)$,
% for any path cyclic $p \in P$,
for any path $p$ longer than $l$,
the condition $\CB_{10}$ states that 
reducing 
the value of $p$ with
the value of $\simple(p)$
leaves the value of $\simple(p)$ unchanged.
Thus,
$
\undersetp{
    p \, \in \, P^k(v)
}{\R} \, \F(p)
=
\undersetp{
    p \, \in \, P^{l+1}(v)
}{\R} \, \F(p)
$.
Thus,
$
\aSpec^{k}(v) 
= 
\{ 
\undersetp{
    p \, \in \, P^{l+1}(v)
}{\R} \, \F(p)
\}
$.
Similarly, it can be shown that
$
\Spec(v) 
= 
\{ 
\undersetp{
    p \, \in \, P^{l+1}(v)
}{\R} \, \F(p)
\}
$.
Therefore,
$\aSpec^{k}(v) = \{ \Spec(v) \}$.



% The computation stops when the values of the vertices stay the same in two consecutive iterations.


An immediate corollary of the above theorem is that 
if the graph is acyclic or the condition $\CB_{10}$ holds,
then all the four asynchronous iteration models eventually terminate and converge to the specification
(if their corresponding conditions in 
\autoref{thm:a-iteration-pull-app} to
\autoref{thm:a-iteration-push-noni-app} hold).
% 
For example the corollary for the asynchronous pull model for idempotent reduction functions is the following. The corollary for the other models is similar.


\begin{corollary}[Termination]
\label{cor:a-iteration-pull}
Forall $\R$, $\F$, $\C$, $\I$, and $\P$,
if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_9$ hold
and
the graph is acyclic or the condition $\CB_{10}$ holds,
then there exists an iteration $k$ such that
$
\S_\apulli^k(v) = 
\Spec(v)
$
\end{corollary}




\clearpage
\subsubsection{Streaming Graphs}
\ \ \ 

\label{sec:streaming-graphs}
In contrast to a static graph,
a streaming graph can continuously change in response to external events.
% 
Thus, 
to have up-to-date results,
the graph analytics computations should be periodically repeated.
% after updates.
% 
Stream graph processing strives to
benefit from the results computed prior to the updates
instead of restarting the iteration form the initial values.
% 
The idea is that starting from the prior result
can accelerate the convergence.
% 
What are the conditions such that
% under which 
% The question is whether 
the incremental computation yields the correct results?
% 
We first consider addition and then removal of edges
and present the correctness conditions 
for incremental commutation after each.




\textbf{Incremental Computation. }
% 
Consider a graph $G$.
Let us denote
the result of a path-based reduction $\Spec(v)$ on $G$
as $\Spec_G(v)$.
% 
% Let $G + \delta$ be 
Let $G + \delta$ be 
the result of updating (adding or removing) an edge $e = \<s_e, t_e\>$
% applying updates to 
in $G$.
% 
The incremental computation 
% of $\Spec(v)$ 
on $G + \delta$
starts from the prior result $\Spec_G(v)$ for $G$.
% of the computation.
% 
The incremental 
pull model 
% (with idempotent reduction) can be defined as follows.
% 
% It 
is similar to 
the basic model
(of \autoref{def:computation-pull}).
The difference is that (1)
the starting state is $\Spec_G(v)$ instead of $\I(v)$ except for the sink node $t_e$ and if the update is a removal,
and 
% that the first active vertex is $v_e$.
(2) that the vertex $t_e$ is updated in the starting iteration.
% 
% Let $\S_{G + \delta}^k(v)$ denote the result of 
Thus, the state of the
% result of 
incremental computation at iteration $k$
denoted as 
$\S_{G + \delta}^k(v)$
is defined as follows:
% (In this definition, the change in the value of $s_e$ from the iteration $0$ to $1$
% causes the update for the value of $t_e$ in the iteration $2$.)
% 
% 
% 
\begin{definition}[Incremental pull model (with idempotent reduction)]
\label{def:computation-pull-inc}
% \ \\ \t
$$
\small
\begin{array}{lcll}
% \S_{G + \delta}^0(v)  & \coloneqq & 
% % \bot
% \twopartdef{
%     \bot
% }{
%     v = s_e
% }{
%     \Spec_G(v)
% }
% \ \\
\S_{G + \delta}^1(v)  & \coloneqq &
% \I(v)
% \Spec_G(v)
\twopartdef{
    \I(v)
}{
   (\delta \mbox{ is removal}) \land (v = t_e)
}{
   \Spec_G(v) 
}
\ \\
\S_{G + \delta}^{k+1}(v)  & \coloneqq &
\twopartdef{
    \R \left[
        \S_{G + \delta}^k(v), \ 
        \undersetp{ \, u \in \preds(v) }{\R}
%         \left( 
        \, \P \! \left( \S_{G + \delta}^k(u), \<u, v\> \right)
%         \right)
    \right]
}{
    (k = 1 \land v = t_e)
    \lor
    (\CPreds^k(v) \neq \emptyset)
}{
    \S_{G + \delta}^k(v)
}
&
\!\!\!\!\!\!\!
k \geq 1
\end{array}
$$
\end{definition}



\textbf{Addition of Edges. }
% 
If the update $\delta$ in $G + \delta$ is adding an edge,
% $\<s_e, t_e\>$,
does the result of incremental computation 
$\S^k_{G + \delta}(v)$
converge to its specification 
% $\Spec_{G + \delta }(v)$?
$\Spec(v)$?
% 
It turns out that it does with the same conditions as the static case.
% The reason is that
Adding an edge only increases the set of paths.
The prior value of a vertex is the result of reduction on the old set of paths to that vertex.
That set may now be incomplete.
However, the prior values can help the incremental computation skip most of the initial iterations.
% 
For example, in the shortest path $\SSSP$ use-case,
the newly added edge may 
% or may not 
improve 
% result in shorter paths for some vertices.
% However, it may not improve 
the previously found shortest path only for some of the vertices.
% that is found for a vertex.
% for other vertices.
% 
Subsequent iterations will eventually reduce 
the values of all the new paths with 
the prior values of the vertices.
% 
As the reduction function is assumed to be commutative, associative and idempotent,
the reduction order 
and
% is not important
% and as it is assumed to be idempotent,
% reducing a path more than once 
repeated reductions of a path 
% value
do not affect the result.
% 
Thus, we can state the following theorem 
for the correctness of incremental reduction after adding edges.



\begin{theorem}[Correctness after adding edges]
\label{thm:iteration-termination-add-inc-app}
% \ \\ \t
For all $\R$, $\F$, $\I$ and $\P$,
% the graph is acyclic or
% the condition $\CB_{10}$ holds, 
% if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_{10}$ hold
if the conditions $\CB_1$ - $\CB_{10}$ hold
and the update $\delta$ is addition of an edge,
then
there exists $k$ such that 
% for every $k' \geq k$,
% \ \\ \t
$\S_{G + \delta }^{k}(v) = \Spec(v)$.
% there exists $k$ such that
% % \ \\ \t
% $\Spec^{k}(v) = \Spec^{k +1}(v) = \Spec(v)$.
\end{theorem}

% \ftom{I think in the removal, the value of the $t_e$ must always reset to the initial value. 
% \autoref{def:computation-pull-inc} will be changed to this:
% \begin{definition}[Incremental pull model (with idempotent reduction)]
% \label{def:computation-pull-inc}
% % \ \\ \t
% $$
% \small
% \begin{array}{lcll}
% % \S_{G + \delta}^0(v)  & \coloneqq & 
% % % \bot
% % \twopartdef{
% %     \bot
% % }{
% %     v = s_e
% % }{
% %     \Spec_G(v)
% % }
% % \ \\
% \S_{G + \delta}^1(v)  & \coloneqq &
% % \I(v)
% % \Spec_G(v)
% \twopartdef{
%     \Spec_G(v)
% }{
%    \delta : \mathsf{addition}
% }{
%     \I(v)
% }
% &
% \!\!\!\!\!\!\!
% \ \\
% \S_{G + \delta}^{k+1}(v)  & \coloneqq &
% \twopartdef{
%     \R \left[
%         \S_{G + \delta}^k(v), \ 
%         \undersetp{ \, u \in \preds(v) }{\R}
% %         \left( 
%         \, \P \! \left( \S_{G + \delta}^k(u), \<u, v\> \right)
% %         \right)
%     \right]
% }{
%     (k = 1 \land v = t_e)
%     \lor
%     (\CPreds^k(v) \neq \emptyset)
% }{
%     \S_{G + \delta}^k(v)
% }
% &
% \!\!\!\!\!\!\!
% k \geq 1
% \end{array}
% $$
% \end{definition}
% }


% \begin{wrapfigure}[18]{R}{0.5\textwidth}
% \begin{wrapfigure}{R}{0.5\textwidth}
\begin{figure}
\centering
%\begin{figure}[t]
\begin{subfigure}{.4\textwidth}
\centering
\includegraphics[scale=0.35]{figures/TextFig/out/C_stream-remove-edge-a.pdf}
\caption{Removing an edge and the subsequent update through a cycle}
\label{fig:stream-a}
\end{subfigure}
% 
\ \ \ \ 
% 
\begin{subfigure}{.4\textwidth}
\centering
\includegraphics[scale=0.35]{figures/TextFig/out/C_stream-remove-edge-b.pdf}
\caption{Removing an edge in the $\CC$ use-case}
\label{fig:stream-b}
\end{subfigure}
% \caption{Illustration of the pull model and its correctness}
\caption{Removing edges}
\label{fig:streaming}
%\end{figure}
% \end{wrapfigure}
\end{figure}


\textbf{Removal of Edges. }
% 
In contrast to adding, 
if the update is removing an edge,
the incremental computation is not necessarily correct.
% 
When an edge $\<s_e, t_e\>$ is removed, 
the value of $t_e$ becomes incorrect 
if it 
% the value of $t_e$ 
has been calculated using the value of $s_e$.
% 
Thus, the incremental computation (\autoref{def:computation-pull-inc}) recalculates the value of $t_e$ based on the values of its remaining predecessors.
% 
The intention is that this update calculates the correct value of $t_e$. 
However, 
as \autoref{fig:stream-a} shows,
if there is a loop from $t_e$ back to one of its predecessors $u$,
and the value of $u$ has been calculated based on the old value of $t_e$,
the recalculated value of $t_e$ is still incorrect.
% 
The new value of $t_e$ can lead to calculation of new values back to $u$ and then again for $t_e$.
% 
The question is whether the iterative calculation around the loop eventually forgets the incorrect value.
% 
It turns out that it does, 
% but
if extending a path with an edge makes the value of the path less favorable during reduction.
%
For example, in the $\SSSP$ use-case,
the value of a path is its weight and
the weight of an extended path increases;
thus, the extended path 
is less favorable for the $\min$ reduction function.
% 
The cycle can take only larger values back to $t_e$ through the predecessor $u$,
and eventually, the values coming from the other predecessors will be smaller
and thus, chosen by the $\min$ reduction function.
% 
% For example,
Thus,
the incremental computation
for
the shortest path use-case $\SSSP$ will eventually converge to the correct values.
 

% \begin{figure*}
% \begin{figure*}[h!]
% \begin{wrapfigure}[28]{R}{0.5\textwidth}
\begin{wrapfigure}{R}{0.5\textwidth}
% \begin{wrapfigure}[29]{R}{0.5\textwidth}
% \begin{wrapfigure}[31]{R}{0.5\textwidth}
% \begin{wrapfigure}[32]{R}{0.5\textwidth}
\small

% \noindent
$
\begin{array}{l}

\mbox{Streaming:}
\ \\ \t
\CB_{12} \ (\mbox{Worsening})\colon 
\\ \t\t
\forall p, e. \ 
\R(\F(p), \F(p \cdot e)) = \F(p) \neq \F(p \cdot e)

\end{array}
$


\caption{
%     Iteration 
    Correctness and Termination Conditions
}
\label{fig:correct-conds-app}
% \end{figure*}
\end{wrapfigure}


However, in the $\CC$ use-case,
the value of a path is
the identifier of its source;
thus, the value of an extended path stays the same.
% 
Consider the graph in \autoref{fig:stream-b} where two cycles are connected by the edge $e = \<s_e, t_e\>$
where the cycle on the $s_e$ side has the vertex with the smallest identifier $0$.
The iteration for $G$ results in $0$ as the component identifier of all vertices.
% (Let us consider an undirected edge as two directed edges.)
Upon the removal of $e$,
the neighbors $u$ of $t_e$ in the loop continue feeding $0$ back to $t_e$ which prevents spreading the larger identifier $4$ in the cycle.
Vertices adopt smaller identifier from their neighbors.
The iteration incorrectly converges to $0$ as the component identifier of the cycle.
% 
We have captured the above sufficient condition 
in \autoref{fig:correct-conds-app}
as the worsening property $\CB_{12}$.
% 
Extending a path $p$ with an edge $e$ should result in an unequal and worse value.
% 
Thus, we can state the following theorem
for the correctness of incremental reduction after removing edges.


\begin{theorem}[Correctness after removing edges]
\label{thm:iteration-termination-remove-inc-app}
% \ \\ \t
For all $\R$, $\F$, $\I$ and $\P$,
% the graph is acyclic or
% the condition $\CB_{10}$ holds, 
% if the conditions $\CB_1$ - $\CB_4$ and $\CB_6$ - $\CB_{11}$ hold
if the conditions $\CB_1$ - $\CB_{10}$ and $\CB_{12}$ hold
and the update $\delta$ is removal of an edge,
then
there exists $k$ such that 
$\S_{G + \delta }^{k}(v) = \Spec(v)$.
\end{theorem}


However, if the condition $\CB_{12}$ does not hold,
then all the prior values cannot be simply used and
the value of all vertices that are reachable form the vertex $t_e$
should be reset to their initial values.
In the example of the \irule{CC} use-case above,
the values of the vertices in the cycle are all reset to their own identifiers.
The iteration then correctly converges to the smallest identifier in the cycle.
% 
As an optimization, 
the dependencies between the value of vertices can be tracked at runtime
and the values of only the vertices that are dependent on $t_e$ should be reset.




\clearpage
\subsubsection{Factored Path-based Reductions}
\label{sec:factored-path-based-red}
\hfill\\
Consider the factored path-based reduction $\underset{c}{\R} \ \F$ with a general configuration $c$.
We show that the correctness conditions for its iterative execution are captured by
the conditions that were presented in \autoref{fig:correct-conds}.
% it can be reduced to  


 
Let us define $C^c$ as follows:
\begin{equation}
% $$
\begin{array}{rcl}
\C^s(p) & \coloneqq & \head(p) = s
\\
\C^\bot(p) & \coloneqq & \True
\end{array}
\label{eq:c-conds-1}
\end{equation}
% $$
Let us define $\F^c$ as follows:
% 
% $$
\begin{equation}
\begin{array}{rcl}
\<\F_1, \F_2\>^{\<c_1, c_2\>}(p) & \coloneqq & \< \F_1^{c_1}(p), \F_2^{c_2}(p) \>
\\
\F^c(p) 
& \coloneqq &
\lif \ (\C^c(p)) \ \F(p) \ \lelse \ \bot
\end{array}
% $$
\label{eq:c-conds-2}
\end{equation}
The specification of the factored path-based reduction $\underset{c}{\R} \ \F$ is the following:
% 
% \begin{definition}[Specification]
% \begin{equation}
% \label{def:red-spec-c-app}
% \begin{array}{l}
$$
% \Spec(v) = 
% \displaystyle
% \underset{p \in \Paths(v) \; \land \; \C(p)}{\R} \F(p)
% \R_{ p \, \in \, \{p \, | \, p \in \Paths(v) \} } \ \F^c(p)
\R_{ p \, \in \Paths(v) } \ \F^c(p)
$$
% \end{array}
% \end{equation}
% \end{definition}
that can be captured by the specification $\Spec(v)$ defined in \autoref{def:red-spec} 
with $\C(p)$ instantiated with $\True$
and $\F$ instantiated with $\F^c$.



Thus, the correctness conditions for the factored path-based reduction
$\underset{c}{\R} \ \F$
can be captured by the conditions that were presented in \autoref{fig:correct-conds}
with $\C(p)$ instantiated with $\True$
and $\F$ instantiated with $\F^c$.
In particular, the initialization condition $\CB_2$ is trivial and $\CB_1$ is simplified to
% $$
\begin{equation}
\I(v) = \F^c(\<v,v\>)
\label{eq:c-conds-3}
\end{equation}
For example, 
by \autoref{eq:c-conds-3} and \autoref{eq:c-conds-2},
for a path-based reduction
$\underset{\<c_1, c_2\>}{\R} \ \<\F_1, \F_2\>$,
the initialization conditions are the following
% 
\begin{equation}
\begin{array}{l}
\forall v. \ 
\C^{c_1}(\<v, v\>) \rightarrow \mathsf{fst}(\I(v)) = \F_1(\<v, v\>)
\\
\forall v. \ 
\lnot \C^{c_1}(\<v, v\>) \rightarrow \mathsf{fst}(\I(v)) = \bot
\\
\forall v. \ 
\C^{c_2}(\<v, v\>) \rightarrow \mathsf{snd}(\I(v)) = \F_2(\<v, v\>)
\\
\forall v. \ 
\lnot \C^{c_2}(\<v, v\>) \rightarrow \mathsf{snd}(\I(v)) = \bot
\label{eq:c-conds-4}
\end{array}
\end{equation}
This means that the initialization for each element of the state tuple mirrors the initialization conditions $\CB_1$ and $\CB_2$.




\clearpage
\subsection{Synthesis of Iterative Reduction}
\label{sec:synthesis-app}





To find candidate expressions for the body of the kernel functions,
% for the body of the iteration functions.
we apply a type-guided enumerative search
to the expression grammar presented
% in \autoref{fig:enum-process-app}.(c).
in \autoref{fig:enum-process-app}b.
% 
The expression constructors have union types;
for example, the plus operator $+$ can be applied to both integers $\mathsf{Int}$ and floating point $\mathsf{Float}$ numbers.
% 
%
% that is represented as 
The procedure $\mathsf{Candidates}$
% in \autoref{fig:enum-process-app}.(a).
in \autoref{fig:enum-process-app}a
% 
% Given a type $T$ and a size $\mathit{size}$,
returns the set of expressions of the input type $T$ and size $\mathit{size}$.
% from 
% input $size$ indicate the depth of the AST.
% enumerates and 
% 
% 
% $\mathsf{Candidates}$ 
It is a recursive procedure that uses memoization to avoid redundant enumeration.
It keeps a map from types to maps from sizes to the set of previously synthesized expressions. 
% (that is not shown in \autoref{fig:enum-process-app}.(a)).
% previously enumerated expressions 
% 
To synthesize an expression of type $T$,
% the $\mathsf{Candidates}$ procedure 
it only considers the expression constructors with the return type $T$.
A constructor itself uses one unit of size.
For each constructor $c$,
the $\mathsf{Candidates}$ procedure considers all the possible distributions of the remained size, that is $\mathit{size} - 1$, between the parameters of $c$. 
For each distribution,
it recursively obtains a set of expressions $E_i$ for each parameter $p_i$
using its type and its allocated size.
It then applies $c$
% the constructor
to each element of the product of the sets $E_i$
to yield candidate expressions.
It memoizes and returns the set of these candidates.







The functions \autoref{fig:enum-process-app}c and \autoref{fig:enum-process-app}d
synthesize the functions $\I$ and $\P$.
We consider synthesis for $\P$; synthesis for $\I$ is similar.
% 
% \autoref{fig:enum-process-app}.(b)
\autoref{fig:enum-process-app}d
presents the $\mathsf{Synth}\P$ procedure that 
given the path function $\F$ and the reduction function $\R$ 
of a path-based reduction,
synthesizes the propagation function $\P$.
% 
% (The synthesis of the initialization function $\I$ is similar 
% and is available in 
% the appendix \autoref{sec:synthesis-app}.)
% \appref{\secSynthesisApp}.)
%  
It 
% The procedure $\mathsf{Synth}\P$ 
% first memoizes
starts by memoizing
expressions of size one, variables and literals,
to make them available for the synthesis of the body of $\P$.
% 
% It 
% % first 
% memoizes all the literals of the grammar.
% 
% The initialization function $\I$ takes a vertex as input and
% returns a value of the return type of $\F$.
Let $T$ be the return type of $\F$;
vertices store values of type $T$.
% 
The propagation function $\P$ takes 
a value stored at a vertex (of type of $T$)
and an edge (of type $\mathsf{Edge}$)
and returns a vertex value (of type $T$).
%
Thus, the two input variables of the two input types,
the variable $n$ of type $T$ 
% the return type of $\F$
and
the variable $l$ of type Edge,
are 
memoized as available expressions.
% the propagation function.
% are memoized.
% 
Then,
candidate expressions of type $T$
% the return type of $\F$
are obtained from the $\mathsf{Candidates}$ procedure.
% 
Expressions of larger sizes are incrementally checked 
as candidate bodies for $\P$.
% the propagation function.


% To synthesize the initialization function, $\I$, we closely follow the method in \autoref{fig:init-synth}.
% It presents the $\mathsf{Synth}\I$ procedure that 
% given the path function $\F$ 
% synthesizes the initialization function $\I$.
% %  
% The initialization function $\I$ takes a vertex as input and
% returns a value of the return type of $\F$ as the initial value of the vertex.
% %
% The procedure $\mathsf{Synth}\I$ 
% % first memoizes
% starts by memoizing
% expressions of size one, literals and variables,
% to make them available for the synthesis of the body of $\I$.
% % 
% % It 
% % % first 
% % memoizes all the literals of the grammar.
% % 
% % The initialization function $\I$ takes a vertex as input and
% % returns a value of the return type of $\F$.
% Let $T$ be the
%  return type of $\F$.
% vertices store values of type $T$.
% Then,
% candidate expressions of type $T$
% % the return type of $\F$
% are obtained from the $\mathsf{Candidates}$ procedure.
% % 
% Expressions of larger sizes are incrementally checked 
% as candidate bodies for $\P$.
% %
% A candidate initialization function $\lambda v. \ e$ is correct if the conditions $\CB_1$ and $\CB_2$  are valid when $\I$ is replaced
% by the candidate function.




% The correctness of 
A candidate propagation function 
$\lambda n, l. \ e$ 
is correct if
% is checked
% by the validity of 
% the conditions $\CB_3$ and 
the conditions
$\CB_4$ 
and
$\CB_5$ 
are valid
% is valid
when $\P$ is replaced by the candidate.
% 
% 
We use the notation of $\mathcal{A} \envof \mathcal{A}'$ to represent 
whether the assertion $\mathcal{A}'$ is valid in the context of 
the assumed assertion(s) $\mathcal{A}$.
To check the validity of an assertion,
we use off-the-shelf SMT solvers to check the satisfiability of its negation.
% 
The context of the validity check
$\F; \R; \Gamma$
is
the definition of the functions $\F$ and $\R$ from the given path-based reduction,
and
a set of assertions $\Gamma$ 
that define basic graph functions and relations.
% 
% axiomatize that defining 
% \autoref{fig:enum-process-app}.(d)
%Here we present the context assertions for the known path functions in graph processing domain.


\autoref{fig:synth-context-app} represents the context assertions $\Gamma$:
% 
% \autoref{fig:enum-process-app}d
assertions for the path functions
$\mathsf{length}$, 
$\mathsf{weight}$, $\mathsf{punultimate}$ and $\mathsf{capacity}$.
% 
% (All assertions of the context $\Gamma$ are available in 
% the appendix \autoref{sec:synthesis-app}.)
% \appref{\secSynthesisApp}.)
% 
We define graph functions and relations in 
the combination of the quantified uninterpreted functions and list theories.
We represent a path $\PathSet$ as a list of vertices $\V$.
The edge weight $\mathsf{eweight}$ is a function on pairs of vertices $\<\V, \V\>$
and
the path weight $\mathsf{weight}$ is a function on paths $\PathSet$ to natural numbers $\Nat$.
% 
% We define 
% The edge weight of loops 
% % to be 
% is
% zero.
% 
If the list for the path is empty or has a single vertex,
% we define 
the weight of the path is trivially zero;
otherwise,
the weight of the path is recursively
the sum of 
% the weight of the rest of the path
the weight of the path without the last edge
and
the edge weight of the last edge.



For the push model with non-idempotent reduction (\autoref{def:computation-push-noni-opt-text}),
% For synthesis in this model,
after the propagation function $\P$ is synthesized,
the condition $\CB_{11}$ is used to synthesize the rollback function $\B$.


We note that since the path functions $\F$ never return none $\bot$,
the reduction function $\R'$ is simplified to $\R$ in
% the conditions $\CB_3$ and $\CB_4$.
the condition $\CB_4$.




\begin{figure}[h!]
\centering
\small
$
\begin{array}{ll}

\begin{array}{l}
\\
%\multicolumn{2}{l}{
\textsf{\textsf{def }} \mathsf{Candidates}(T, \mathit{size})
%}
\\ 
\ \ \ \lif \ (\mbox{already memoized $E$ }
\\
\ \ \ \phantom{\ \ \ \lif}
            \mbox{for $T$ and $\mathit{size}$})
\\
\ \ \ \ \ \ \lreturn \ E
\\
\ \ \ E \leftarrow \emptyset
\\
\ \ \ \lforeach \ (\mbox{expression constructor $c$}
\\
\ \ \ \phantom{\lif}
            \mbox{with the return type $T$})
\\ 
\ \ \ \ \ \ \lforeach \ (\mbox{distribution $\overline{s_i}$ of $\mathit{size}-1$}
\\
\ \ \ \phantom{\ \ \ \lif}
            \mbox{between parameters $\overline{p_i}$ of $c$})
\\ 
\ \ \ \ \ \ \ \ \ \lforeach \ (\mbox{$p_i$ with type $T_i$})
\\
\ \ \ \ \ \ \ \ \ \ \ \ E_i \leftarrow \mathsf{Candidates}(T_i, s_i)
\\
\ \ \ \ \ \ \ \ \ E \leftarrow E \union \{ c(\overline{e}) \ | \ \overline{e} \in \times \, \overline{E_i} \}
\\
\ \ \ \mbox{memoize $E$ for $T$ and $\mathit{size}$}
\\
\ \ \ \lreturn \ E
\\[1ex]
% \\
%\multicolumn{2}{c}{
    \mbox{\ \ (a) Type-guided expression}
    \\
        \mbox{\t \t \ \ \ enumeration}
%}
\end{array}

&

\begin{array}{rcl@{\qquad}l}
      e
         & ::= &
            n
            \ \ | \ \
            v
        &
            \!\!\!\!\!\!
%             \mbox{Expression}
            \mbox{Exp}
    \\
    
         & | &
            e+e
            \ \ | \ \
            e-e
            
    \\      
%       c
%          & ::= &
         & | &
            e = e
            \ \ | \ \
            e < e
         &
%          \!\!\!\!\!\!
%          \mbox{Condition}   

    \\
         & | &
            \min(e,e)
            \ \ | \ \
            \max(e,e)

    \\
         & | &
            \lif \ (e) \lthen e \ \lelse \ e
         &
            \!\!\!\!\!\!
%             \mbox{Constructors}
    \\
         & | &
            \mathsf{weight}(e)
            \ \ | \ \
            \mathsf{capacity}(e)
            
    \\
    &| &
            \mathsf{indeg}(e)
            \ \ | \ \
            \mathsf{outdeg}(e)
            
    \\
         & | &
            \mathsf{src}(e)
            \ \ | \ \
            \mathsf{dst}(e)
%             \ \ | \ \
         &
         \!\!\!\!\!\!
    \\
         & | &
        |V|
    \\    
         n
         & ::= &
            0
            \ \ | \ \
            1
            \ \ | \ \
            ..
            \ \ | \ \
            \True
            \ \ | \ \
            \False
         &
         \!\!\!\!\!\!
         \mbox{Literal}
    \\    
         v
         &  &
         &
         \!\!\!\!\!\!
         \mbox{Variable}
    \\
            T
         & ::= &
         \mathsf{Int}
         \ \ | \ \ 
         \mathsf{Float}
         \ \ | \ \ 
         \mathsf{Bool}
         \ \ | \ \ 
    \\    
    &&
         \mathsf{Edge}
         \ \ | \ \ 
         \mathsf{Vertex}
         &
         \!\!\!\!\!\!
         \mbox{Type}
      \\[1ex]
%       \\   
      \multicolumn{4}{c}{\mbox{(b) Grammar} }
   \end{array}

\\

\begin{array}{ll}
\\
\multicolumn{2}{l}{
\textsf{def } \mathsf{Synth}\I \, (\F)
}
\\ 
I_1  & \mbox{memoize the variable $v$ for type $\mathsf{Vertex}$ and size $1$} 
\\
I_2  & \lforeach \ (\mbox{literal $l_i$ with type $T_i$})
\\
I_3  & \t \mbox{memoize $l_i$ for $T_i$ and size $1$} 
\\
I_4  & \mathit{size} \leftarrow 1
\\
I_5  & \mathsf{while} \ (\true)
\\
I_6  & \t E \leftarrow \mathsf{Candidates}(\mbox{return type of $\F$, $\mathit{size}$})
\\
I_7 & \t \lforeach \ (e \in E)
\\
% I_8 & \t\t \lif \ \F; \Gamma \vdash \{\CB_1 \land \CB_2\}[\I \mapsto (\lambda v. \ e)]
I_8 & \t\t \lif \ \F; \Gamma \vdash (\CB_1 \land \CB_2) [\I \mapsto (\lambda v. \ e)]
\\
I_9 & \t\t\t \lreturn \ (\lambda v. \ e)
\\
I_{10}  & \t \mathit{size} \leftarrow \mathit{size} + 1
\\[1ex]
%       \\   
\multicolumn{2}{c}{\mbox{(c) Synthesis of the initialization function $\I$} }
\end{array}

&

\begin{array}{ll}
\\
\multicolumn{2}{l}{
\textsf{def } \mathsf{Synth}\P \, (\F, \R)
}
\\
        & \mbox{let $T$ be the return type of $\F$.}
\\
P_1  & \mbox{memoize variable $n$
% }
% \\
%         & \t 
%         \mbox{
        for $T$ and size $1$}
\\
P_2  & \mbox{memoize variable $l$
% } 
% \\
%         & \t 
%         \mbox{
        for type $\mathsf{Edge}$ and size $1$}
\\ 
P_3  & \lforeach \ (\mbox{literal $l_i$ with type $T_i$})
\\
P_4  & \t \mbox{memoize $l_i$ for $T_i$ and size $1$} 
\\
P_5  & \mathit{size} \leftarrow 1
\\
P_6  & \mathsf{while} \ (\true)
\\
P_7  & \t E \leftarrow \mathsf{Candidates} \,(T, \mathit{size})
\\
P_8 & \t \lforeach \ (e \in E)
\\
% P_9 & \t\t \lif \ \F; \R; \Gamma \vdash (\CB_3 \land \CB_4) [\P \coloneqq (\lambda n, l. \ e)]
P_9 & \t\t \lif \ \F; \R; \Gamma \vdash (\CB_4 \land \CB_5) [\P \coloneqq (\lambda n, l. \ e)]
\\
P_{10} & \t\t\t \lreturn \ (\lambda n, l. \ e)
\\
P_{11}  & \t \mathit{size} \leftarrow \mathit{size} + 1
\\[1ex]
% \\
\multicolumn{2}{c}{
    \mbox{(d) Synthesis of the propagation function $\P$}
}
\end{array}

\end{array}
$

\caption{Synthesis Grammar and functions}
\label{fig:enum-process-app}
\end{figure}





% \clearpage





% \begin{array}{l@{}}
% \\
% \textsf{fun } \I\mathsf{Synth}(\mathcal{G} \ G,\textsf{M} \ m, \textsf{Int} \ limit) \{% \colon \mathcal{G} \ \times  \ \Nat \rightarrow \mathsf{Program} \ \{
% \\ 
% C_1  \t \lforeach ( \R \ \F \in m)
% \\ 
% C_2  \t\t \mathsf{E} \leftarrow \{e | e \in G.terminals \}
% \\ 
% C_3  \t\t \mathsf{size} \leftarrow 1
% \\ 
% %C_4  \t\t \textsf{var} \ \mathsf{ISig} \colon \V \rightarrow \F.rtype 
% %\\ 
% C_4  \t\t \textsf{var} \ \I \colon \V \rightarrow \F.rtype 
% \\
% C_5  \t\t \mathsf{while} \ \mathsf{size} < limit \ \mathsf{do} \colon
% \\ 
% C_6  \t\t\t p \leftarrow E.\mathsf{next()}
% \\
% C_7  \t\t\t \Gamma \coloneqq \R;\F;p
% \\
% C_8  \t\t\t \lif \ \Gamma \vdash \{\CB_1 - \CB_2\}[\I \mapsto p]
% \\ 
% C_9  \t\t\t\t \I \coloneqq p
% \\
% C_{10} \t\t\t\t \mathsf{break}
% \\ 
% C_{11} \t\t\t\ E \leftarrow E \cup \mathsf{addExp(G, \I.type)}
% \\ 
% C_{12} \t\t\t \mathsf{size} \leftarrow \mathsf{size} + 1
% \\\\
% \t\t\t\t\t\mbox{(a)}
% \end{array}
% 
% &
% 
% \begin{array}{l@{}}
% \\
% \textsf{fun } \P\mathsf{Synth}(\mathcal{G} \ G,\textsf{M} \ m, \textsf{Int} \ limit) \{% \colon \mathcal{G} \ \times  \ \Nat \rightarrow \mathsf{Program} \ \{
% \\ 
% C_3  \t \lforeach ( \R \ \F \in m)
% \\ 
% C_1  \t\t \mathsf{E} \leftarrow \{e | e \in G.terminals \}
% \\ 
% C_2  \t\t \mathsf{size} \leftarrow 1
% %C_4  \t\t \textsf{var} \ \mathsf{ISig} \colon \V \rightarrow \F.rtype 
% %\\ 
% \\
% C_4  \t\t \textsf{var} \ \P \colon
% % \\ \t\t\t\t
% \F.rtype \times \mathsf{E}.type \rightarrow \F.rtype 
% \\
% C_5  \t\t \mathsf{while} \ \mathsf{size} < limit \ \mathsf{do} \colon
% \\ 
% C_6  \t\t\t p \leftarrow E.\mathsf{next()}
% \\
% C_7  \t\t\t \Gamma \coloneqq \R;\F;p
% \\
% C_8  \t\t\t \lif \ \Gamma \vdash \{\CB_3 - \CB_4\}[\P \mapsto p]
% \\ 
% C_9  \t\t\t\t \P \coloneqq p
% \\
% C_{10}  \t\t\t\t \mathsf{break}
% \\ 
% C_{11}  \t\t\t\ E \leftarrow E \cup \mathsf{addExp(G, \P.type)}
% \\ 
% C_{12} \t\t\t \mathsf{size} \leftarrow \mathsf{size} + 1
% \\\\
% \t\t\t\t\t\mbox{(b)}
% \end{array}



\begin{figure}[h!]
\centering
\small
% \resizebox{.85\textwidth}{!}{
$
\begin{array}{rcl}
\begin{array}{l@{}}
\Gamma =
\end{array}
&
\begin{array}{l@{}}
\PathSet \coloneqq \List[\V],
\\
\\
\mathsf{length} \colon \PathSet \rightarrow \Nat
\\
\mathsf{elength} \colon \<\V, \V\> \rightarrow \Nat
\\
\forall \<u, v\>. \ 
% \in \PathSet. 
% \\ \t
    \lif \ (u = v) \ \ 
% \\ \t\t
        \mathsf{elength}(\<u, v\>) = 0
\\ \t
    \lelse
\\ \t\t
       \mathsf{elength}(\<u, v\>) = 1 \
\\
\forall p. \ 
% \in \PathSet. 
% \\ \t
    \lif \ (p = \bot) \ \ 
% \\ \t\t
        \mathsf{length}(p) = 0
\\ \t
    \lelse
\\ \t\t
        \llet v \coloneqq \head(p),  p' \coloneqq \tail(p) \lin \
% \\ \t\t
%         \llet v \coloneqq \head(p) \lin \
% \\ \t\t
%         \llet pp \coloneqq \tail(p) \lin \ 
\\ \t\t
    \lif \ (p' = \bot) \ \ 
% \\ \t\t\t
        \mathsf{length}(p) = 0
\\ \t\t
    \lelse
\\ \t\t\t
        \llet v' \coloneqq \head(p') \lin \ 
\\ \t\t\t
        \mathsf{length}(p) = 
\\ \t\t\t \phantom{X}
        \mathsf{length}(p') + \mathsf{elength}(\<v', v\>)
\\
\\
%\multicolumn{1}{c}{
%   \mbox{(d) Context assertions $\Gamma$ (for length)}

\mathsf{penultimate} \colon \PathSet \rightarrow \V
\\
\forall p. \ 
% \in \PathSet. 
% \\ \t
    \lif \ (p = \bot) \ \ 
% \\ \t\t
        \mathsf{penultimate}(p) = \bot
\\ \t
    \lelse
\\ \t\t
        \llet v \coloneqq \head(p),  p' \coloneqq \tail(p) \lin \
% \\ \t\t
%         \llet v \coloneqq \head(p) \lin \
% \\ \t\t
%         \llet pp \coloneqq \tail(p) \lin \ 
\\ \t\t
    \lif \ (p' = \bot) \ \ 
% \\ \t\t\t
        \mathsf{penultimate}(p) = v
\\ \t\t
    \lelse
\\ \t\t\t
        \mathsf{penultimate}(p) = \head(p')
\\
\\
\end{array}
&
\begin{array}{l@{}}
\mathsf{weight} \colon \<\V, \V\> \rightarrow \Nat
\\
\forall v. \ \mathsf{eweight}(\<v, v\>) = 0
\\
\forall p. \ 
% \in \PathSet. 
% \\ \t
    \lif \ (p = \bot) \ \ 
% \\ \t\t
        \mathsf{weight}(p) = 0
\\ \t
    \lelse
\\ \t\t
        \llet v \coloneqq \head(p),  p' \coloneqq \tail(p) \lin \
% \\ \t\t
%         \llet v \coloneqq \head(p) \lin \
% \\ \t\t
%         \llet pp \coloneqq \tail(p) \lin \ 
\\ \t\t
    \lif \ (p' = \bot) \ \ 
% \\ \t\t\t
        \mathsf{weight}(p) = 0
\\ \t\t
    \lelse
\\ \t\t\t
        \llet v' \coloneqq \head(p') \lin \ 
\\ \t\t\t
        \mathsf{weight}(p) = 
\\ \t\t\t \phantom{X}
        \mathsf{weight}(p') + \mathsf{eweight}(\<v', v\>)     
\\
\\
\mathsf{capacity} \colon \PathSet \rightarrow \Nat
\\
\mathsf{ecapacity} \colon \<\V, \V\> \rightarrow \Nat
\\
\forall v. \ \mathsf{ecapacity}(\<v, v\>) = \bot
\\
\forall p. \ 
% \in \PathSet. 
% \\ \t
    \lif \ (p = \bot) \ \ 
% \\ \t\t
        \mathsf{capacity}(p) = \bot
\\ \t
    \lelse
\\ \t\t
        \llet v \coloneqq \head(p),  p' \coloneqq \tail(p) \lin \
% \\ \t\t
%         \llet v \coloneqq \head(p) \lin \
% \\ \t\t
%         \llet pp \coloneqq \tail(p) \lin \ 
\\ \t\t
    \lif \ (p' = \bot) \ \ 
% \\ \t\t\t
        \mathsf{capacity}(p) = \bot
\\ \t\t
    \lelse
\\ \t\t\t
        \llet v' \coloneqq \head(p') \lin \ 
\\ \t\t\t
        \mathsf{capacity}(p) = 
\\ \t\t\t \phantom{X}
        \min(\mathsf{capacity}(p'), \mathsf{ecapacity}(\<v', v\>))
\end{array}
\end{array}
$
% }
\caption{\label{fig:synth-context-app}
    Context assertions $\Gamma$
}
\end{figure}



==> Usecases.tex <==
\clearpage
\section{Use-case Specifications}
\label{sec:use-case-spec-app}

\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}
                     
            \SP(s)(v)& = & % \{
%         \\ \t
          %\forall p \in \Paths(s,v).
          %\\ \t \t
           \displaystyle \min_{  p \in \Paths(s, v)} \weight(p)
           &
           \mbox{Shortest Path}
            \\
            \\

            
            \NP(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
%            \displaystyle \sum_{ p \in \Paths(s,v)} 1
           | \, \Paths(s,v) \, |
            &
            \mbox{Number of Paths}           
            \\
            \\

            \LP(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \displaystyle \max_{ p \in \Paths(s,v)} \weight(p)
            &
            \mbox{Longest Path}
            \\
            \\
            
            \SL(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \displaystyle \min_{ p \in \Paths(s,v)} \length(p)
            &
            \mbox{Shortest Length}
            \\
            \\
            
            \LL(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \displaystyle \max_{ p \in \Paths(s,v)} \length(p)
            &
            \mbox{Longest Length}
            \\
            \\
            
            \WP(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
            \displaystyle \max_{ p \in \Paths(s,v)} \capacity(p)
            &
            \mbox{Widest Path}
            \\
            \\

            
            \NP(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \displaystyle \min_{ p \in \Paths(s,v)} \capacity(p)
           &
           \mbox{Narrowest Path}
            \\
            \\


            
            \FR(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \displaystyle 
           \bigvee_{ p \in \Paths(s,v)} \True
            &
            \mbox{Forward Reachability}
            \\
            \\

            
            \CC(v) & = & 
%             \\ \t \t
%             \displaystyle \min_{p \in \Paths(v)} \id(\head(p))
            \displaystyle \min_{p \in \Paths(v)} \head(p)
            &
            \mbox{Connected Components}
            \\
            \\

            \CCS(v) & = &
            \displaystyle 
            \underset{p \in \Paths(v)}{\bigcup} \{\,\head(p)\,\}
            &
            \mbox{Connected Component Set}
            \\
            \\

            
            \BR(s)(v)& = & % \{
            \displaystyle 
            \bigvee_{ p \in \Paths(v,s)} \True
            &
            \mbox{Backward Reachability}
            \\
            \\

            
            \BFS(s)(v)& = & % \{
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
           \penultimate(\displaystyle \argmin_{ p \in \Paths(s,v)} \length(p))
           &
           \mbox{Breadth-First Search}
            \\
            \\

         \end{array}
      \end{array}
   $
    \caption{\label{fig:benchs-spec-1}
        Use-cases for $\underset{p \in P}{\R} f(p)$ and $f (\underset{p \in P}{\mathsf{arg}\,\R} \,\, f(p))$
    }
% \end{wrapfigure}
\end{figure}

            


\clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}

            \WSP(s)(v) &=&
            \llet P \coloneqq
            \displaystyle \argsmin_{p \in \Paths(s, v)} \length(p)
            \lin            
            &
            \mbox{Widest Shortest Paths}
            \\ &&
            \displaystyle 
                \max_{p \in P}
                    \ 
                    \capacity(p)
            \\
            \\

         
            \NSP(s)(v)& = & % \{
          %\\ \t
          %\forall p \in \Paths(s,v).
%         \\ \t \t
%             \displaystyle 
% %             \sum_{\forall p \in \Paths(s,v)} \length(p) = \SL(s)(v) ? 1 : 0
%             \sum_{p' \in \displaystyle \argsmin_{p \in \Paths(s, v)} \weight(p)} 1
            \left| \, \displaystyle \argsmin_{p \in \Paths(s, v)} \weight(p) \, \right|
            &
            \mbox{Number of Shortest Paths}            
            \\
            \\

            \HLP(v)& = & % \{
            \head(\displaystyle \argmax_{ p \in \Paths(v)} \weight(p))
            &
            \mbox{Head of Longest Path}
            \\
            \\

            \HLL(v)& = & % \{
            \head(\displaystyle \argmax_{ p \in \Paths(v)} \length(p))
            &
            \mbox{Head of Longest Length}
            \\
            \\

            \HNP(v)& = & % \{
            \head(\displaystyle \argmin_{ p \in \Paths(v)} \capacity(p))
            &
            \mbox{Head of Narrowest Path}
            \\
            \\

            \SWSL(s)(v) 
            & = &
            &
                \begin{array}{r}
                \mbox{Shortest Weight in}
                \\
                \mbox{Shortest Length Paths}
                \end{array}
            \\ &&
                \llet P \coloneqq
                \displaystyle \argsmin_{p \in 
                    \Paths(s, v)}
                    \length(p)
                \lin    
            \\ &&
                \displaystyle 
                \min_{p \in P}
                    \ 
                    \weight(p)            
%             \\ &&
%             \displaystyle 
%             \min_{p' \in 
%                 \displaystyle \argsmin_{p \in 
%                 \Paths(s, v)}
%                 \length(p)}
%             \weight(p')
            \\
            \\

            
            \WSLSW(s)(v) & = &
            &
            \begin{array}{r}
            \mbox{Widest in}
            \\
            \mbox{Shortest Length in}
            \\
            \mbox{Shortest Weight Paths}
            \end{array}
            \\ &&
                \llet P \coloneqq 
                \displaystyle 
                \argsmin_{p \in \Paths(s, v)}
                    \weight(p)
                \lin
            \\ &&
                \llet P' \coloneqq 
                \displaystyle
                \argsmin_{p \in P}
                    \length(p)
                \lin
            \\ &&
                \displaystyle 
                \max_{p \in P'}
                    \ 
                    \capacity(p)
%                     
%             \displaystyle 
%             \max_{p'' \in 
%                 \displaystyle 
%                 \argsmin_{p' \in 
%                     \displaystyle \argsmin_{p \in 
%                     \Paths(s, v)} 
%                     \weight(p)}
%                 \length(p')}
%             \capacity(p'')
% 
            \\
            \\


            \LNP(s)(v) & = &
            &
            \mbox{Longest Narrowest Path}
            \\ &&
            \llet P \coloneqq
            \displaystyle 
            \argsmin_{p \in \Paths(s, v)}
                \capacity(p)
            \lin
            \\ &&
            \displaystyle 
            \max_{p \in P}
                \ \length(p)
            \\
            \\


            \HNP(v) & = &
            &
            \mbox{Heads of Narrowest Paths}
            \\ &&
            P \coloneqq
            \displaystyle 
                \argsmin_{p \in \Paths(v)}
                \capacity(p)
            \lin
            \\ &&
            \displaystyle
                \underset{p \in P} 
                {\bigcup}
                \ 
                \{\,\head(p)\,\}
            \\
            \\

            

            \CCSS(v) & = &
%             \\ \t \t
%             \displaystyle \min_{p \in \Paths(v)} \id(\head(p))
%             \displaystyle 
            \left| \, 
            \displaystyle
            \underset{p \in \Paths(v)}{\bigcup} \{\,\head(p)\,\} 
            \, \right|
            &
            \mbox{Connected Component Set Size}
%             \\
%             \\


            
         \end{array}
      \end{array}
   $
   \caption{\label{fig:benchs-spec-33-1}Use-cases for nested $\underset{p \in P}{\R} f(p)$, part 1}
% \end{wrapfigure}
\end{figure}







\clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}


            \NWSP(s)(v) &=&
            &
            \mbox{Number of Widest Shortest Paths}
            \\ &&
            \llet P \coloneqq
            \displaystyle \argsmin_{p \in \Paths(s, v)} \weight(p)
            \lin
            \\ &&
            \llet P' \coloneqq
            \displaystyle \argsmax_{p \in P} \capacity(p)
            \\ &&
            \left| \, P' \, \right|
            \\
            \\


            \NSWSL(s)(v) &=&
            &
            \begin{array}{r}
                \mbox{Number of}
                \\
                \mbox{Shortest Weight in}
                \\
                \mbox{Shortest Length Paths}
            \end{array}
            \\ &&
                \llet P \coloneqq
                \displaystyle \argsmin_{p \in \Paths(s, v)}            
                    \length(p)
                \lin
            \\ &&
                \llet P' \coloneqq
                \displaystyle \argsmin_{p \in P} 
                    \weight(p')
                \lin
            \\ &&
                \left| \, P' \, \right|
            
         \end{array}
      \end{array}
   $
   \caption{\label{fig:benchs-spec-33-2}Use-cases for nested $\underset{p \in P}{\R} f(p)$, part 2}
% \end{wrapfigure}
\end{figure}




\clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}

            \NWR(s)(v)& = & % \{
            \frac{
                \displaystyle 
                \min_{p \in \Paths(s, v)} \capacity(p) 
            }{
                \displaystyle 
                \max_{p \in \Paths(s, v)} \capacity(p) 
            }
            &
            \mbox{Narrowest to Widest Path Ratio}
            \\
            \\


            \LSD(s)(v) &=&
            \LP(s)(v) - \SP(s)(v)
            &
            \begin{array}{r}
                \mbox{Difference between}
                \\
                \mbox{Longest and Shortest Path}
            \end{array}
            \\
            &=&
            \displaystyle 
            \max_{p \in \Paths(s, v)} \weight(p) 
            -
            \displaystyle 
            \min_{p \in \Paths(s, v)} \weight(p) 
            \\
            \\


            \SPTwo(s, s')(v) &=& % \{
%         \\ \t
            %\forall p \in \Paths(s,v).
            %\\ \t \t
%             \displaystyle \min_{  p \in (\Paths(s, v) \, \union \, \Paths(s', v)) } \weight(p)
% 
%             \min(
%               \displaystyle \min_{  p \Paths(s, v) } \weight(p),
%               \displaystyle \min_{  p \in \Paths(s', v) } \weight(p)
%             )
% 
            \min \left(
                \SP(s)(v),
                \SP(s')(v)
            \right)
            &
            \begin{array}{r}
                \mbox{Shortest Path from}
                \\
                \mbox{Two Sources}
            \end{array}
            \\
            
            &=&
                \min \left(
                    \displaystyle 
                    \min_{p \in \Paths(s, v)} \weight(p),
                    \displaystyle 
                    \min_{p \in \Paths(s', v)} \weight(p)
                \right)
            \\
            \\

            \SPR(s, s')(v)&=& % \{
%         \\ \t
            %\forall p \in \Paths(s,v).
            %\\ \t \t
%             \displaystyle \min_{  p \in (\Paths(s, v) \, \union \, \Paths(s', v)) } \weight(p)
% 
%             \min(
%               \displaystyle \min_{  p \Paths(s, v) } \weight(p),
%               \displaystyle \min_{  p \in \Paths(s', v) } \weight(p)
%             )
% 
            \displaystyle 
            \frac{
                \SP(s)(v)
            }{
                \SP(s')(v)
            }
            &
            \begin{array}{r}
                \mbox{Ratio of Shortest Paths}
                \\
                \mbox{from Two Sources}
            \end{array}
            \\
            
            &=&
                \displaystyle
                \frac{
                \displaystyle 
                \min_{p \in \Paths(s, v)} \weight(p) 
            }{
                \displaystyle 
                \max_{p \in \Paths(s', v)} \weight(p) 
            }
            \\
            \\

         \end{array}
      \end{array}
   $
    \caption{\label{fig:benchs-spec-44}
        Use-cases for nested $m \oplus m$
    }
% \end{wrapfigure}
\end{figure}

\clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}
            \ECC(s)& = & % \{
            \displaystyle \max_{v \in \Vertices} 
            \min_{ p \in \Paths(s,v)} \length(p)
            &
            \mbox{Eccentricity}
            \\
            \\
         
            \WPG(s) & = &
            \displaystyle
            \min_{v \in \Vertices}
            \, \WP(s)(v)
            &
            \begin{array}{r}
                \mbox{The Capacity of the Narrowest of}
                \\
                \mbox{the Widest Paths}
                \\
                \mbox{from $s$ to All Vertices}
            \end{array}
            \\
            & = &
          %\\ \t
          % p \in \Paths(s,v).
%         \\ \t \t
            \displaystyle
            \min_{v \in \Vertices}
            \displaystyle 
            \max_{ p \in \Paths(s,v)} \capacity(p)            
            \\
            \\

            
            \LNPG(s) & = &
            \displaystyle
            \max_{v \in \Vertices}
            \, \LNP(s)(v)
            &
            \begin{array}{r}
                \mbox{The Length of the Longest of}
                \\
                \mbox{the Narrowest Paths}
                \\
                \mbox{from $s$ to All Vertices}
            \end{array}
            \\
            &=&            
            \llet P(v) \coloneqq
            \displaystyle 
            \argsmin_{p \in \Paths(s, v)}
                \capacity(p)
            \lin
            \\ &&
            \displaystyle
            \max_{v \in \Vertices}
            \ 
            \displaystyle
            \max_{p \in P(v)}
                \ \length(p)
%             \displaystyle
%             \max_{p' \in 
%                 \displaystyle 
%                 \argsmin_{p \in 
%                 \Paths(s, v)} 
%                 \capacity(p)}
%             \length(p')
            \\
            \\


            \NCC & = & 
            \left| \,
            \displaystyle
            \underset{v \in \Vertices}{\bigcup} 
            \, \CC(v)
            \, \right|            
            &
            \mbox{Number of Connected Components}
            \\
            & = &
            \left| \,
            \displaystyle
            \underset{v \in \Vertices}{\bigcup} 
            \{
            \displaystyle \min_{p \in \Paths(v)} \head(p)
            \}
            \, \right|
            \\
            \\

            
            \FRA(s) & = &
            \displaystyle 
            \bigwedge_{v \in \Vertices}
            \FR(s)(v)
            &
            \mbox{Reachability to All Vertices}
            \\
            & = &
            \displaystyle 
            \bigwedge_{v \in \Vertices}
            \displaystyle 
            \bigvee_{ p \in \Paths(s,v)} \True
            \\
            \\

            
            \RFA & = &
            \displaystyle
            \underset{s \in \Vertices}{\bigcap}
            \, \CCS(s)
            &
            \mbox{Vertices Reachable to All Vertices}
            \\
            & = &
            \displaystyle
            \underset{v \in \Vertices}{\bigcap}
            \,
            \underset{p \in \Paths(v)}{\bigcup} \{\,\head(p)\,\}
%             \\
%             \\

            
         \end{array}
      \end{array}
   $
    \caption{\label{fig:benchs-spec-3}
        Use-cases for $\underset{v \in \Vertices}{\R} m$
    }
% \end{wrapfigure}
\end{figure}


% \clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}
            \\
            \\
         
            \DS(s) & = &
            \displaystyle
            \bigcup_{
                v \in \Vertices \, \land \,
                \SP(s)(v) \, > \, 7
            }
            \{v\}
            &
            \mbox{Vertices with the distance of at least 7}
            \\
            \\
            & = &
            \displaystyle
            \bigcup_{
                v \in \Vertices \, \land \,
                \displaystyle
                \min_{  p \in \Paths(s, v) } 
                \weight(p)
                > 7
            }
            \{v\}
            \\
            \\

            \SCC(s)(v)& = & % \{
            \displaystyle 
            \bigcup_{v' \in \Vertices
            \; \land \;
            \bigvee_{ p \in \Paths(v,v')} \True
            \, \land \,
            \bigvee_{ p \in \Paths(v',v)} \True
            }
            \{ v' \}
            &
            \mbox{Strongly Connected Component}
%             \\
%             \\


        \end{array}
    \end{array}
    $
    \caption{\label{fig:benchs-spec-4}
        Use-cases for 
        $\underset{v \in \Vertices \, \land \, m}{\R} m$
    }
% \end{wrapfigure}
\end{figure}




\clearpage
\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}

            \Radius & = & % \{
            \displaystyle \min_{s \in \{\overline{v}\}} 
            \displaystyle \max_{v \in \Vertices} 
            \min_{ p \in \Paths(s,v)} \length(p)
            &
            \mbox{Radius Sampled on vertices $\{\overline{v}\}$}
            \\
            \\
            
            \Diam & = & % \{
            \displaystyle \max_{s \in \{\overline{v}\}} 
            \displaystyle \max_{v \in \Vertices} 
            \min_{ p \in \Paths(s,v)} \length(p)
            &
            \mbox{Diameter Sampled on vertices $\{\overline{v}\}$}
            \\
            \\


            \DRR & = &
            \displaystyle
            \frac{
                \Diam
            }{
                \Radius
            }
            &
            \mbox{Diameter to Radius Ratio}
            \\
            \\
            & = &
            \displaystyle
            \frac{
                \displaystyle \max_{s \in \{\overline{v}\}} 
                \displaystyle \max_{v \in \Vertices} 
                \min_{ p \in \Paths(s,v)} \length(p)
            }{
                \displaystyle \min_{s \in \{\overline{v}\}} 
                \displaystyle \max_{v \in \Vertices} 
                \min_{ p \in \Paths(s,v)} \length(p)
            }
%             \\
%             \\

        \end{array}
    \end{array}
    $
    \caption{\label{fig:benchs-spec-5}
        Use-cases for $r \oplus r$
    }
% \end{wrapfigure}
\end{figure}



% \begin{figure}[ht!]
% % \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
% %    \figuredefstextsize
%    \small
%    $
% %       \begin{array}{lcl@{\qquad}r}
%       \begin{array}{c}
%          \begin{array}{rclr}
%             
%             &&&
%             \mbox{Betweenness Centrality}
%             \\
% 
%             \rulelabel{BC}
%             \BC(v) & = &
%             \multicolumn{2}{l}{
%                 \displaystyle \sum_{u \in \{\overline{u}\}}
%                 \displaystyle \sum_{
%                 w \in \Vertices \; \land \;
% %                 w \in \{\overline{w}\} \land
%                  \SP(u)(v) \; + \; \SP(v)(w) \; = \; \SP(u)(w)}
%                 \displaystyle
%                 \frac{
% %                     \displaystyle \sum_{}
%                     \NSP(u)(v) \times \NSP(v)(w)
%                 }{
%                     \NSP(u,w)
%                 }
%             }
% 
%             
% %             \rulelabel{BC}
% %             \BC(v) & = &
% %             \multicolumn{2}{l}{
% %                 \displaystyle
% %                 \frac{
% %                     \displaystyle \sum_{u \in \{\overline{u}\}}
% %                     \ \ 
% %                     \displaystyle \sum_{w \in \Vertices \; \land \; \SP(u)(v) + \SP(v)(w) = \SP(u)(w)}
% %                     \NSP(u)(v) \times \NSP(v)(w)
% %                 }{
% %                     \displaystyle \sum_{u \in \{\overline{u}\}}
% %                     \displaystyle \sum_{w \in \Vertices}
% %                     \NSP(u,w)
% %                 }
% %             }
% 
% 
% %             &
% %             \mbox{Betweenness Centrality}
% 
%         \end{array}
%     \end{array}
%     $
%     \caption{\label{fig:benchs-spec-5p}
%         More elaborate Use-cases
%     }
% % \end{wrapfigure}
% \end{figure}






\clearpage

\begin{figure}[ht!]
% \begin{wrapfigure}[22]{R}{0.61\textwidth}  \vspace{-3.5ex}
%    \figuredefstextsize
   \small
   $
%       \begin{array}{lcl@{\qquad}r}
      \begin{array}{c}
         \begin{array}{rclr}

            
            \NPH(s)(v)&=& % \{
          %\\ \t    
          %\forall p \in \Paths(s,v).
%         \\ \t \t
            \displaystyle \sum_{p \in \Paths(s,v)} \length(p) \mapsto 1
            &
            \mbox{Number of Paths Histogram}
            \\
            \\

            
            \LSP(s)(v)&=& % \{
          %\\ \t
          %\forall p \in \Paths(s,v).
%         \\ \t \t
            \displaystyle 
%             \sum_{\forall p \in \Paths(s,v)} \length(p) = \SL(s)(v) ? 1 : 0
            \sum_{p' \in \displaystyle \argsmin_{p \in \Paths(s, v)} \weight(p)} \length(p) \mapsto 1
            &
            \mbox{Length of Shortest Paths}
            \\
            \\
            
            \CCH(v) &=& 
%             \\ \t \t
%             \displaystyle \min_{p \in \Paths(v)} \id(\head(p))
            \displaystyle 
            \sum_{ v \in \Vertices } 
            \displaystyle 
            (\min_{p \in \Paths(v)} \head(p)) \mapsto 1
            &
            \mbox{Connected Components Sizes}
            \\
            \\

            
         \end{array}
      \end{array}
   $
   \caption{\label{fig:benchs-spec-extra}
%         Supported later?
        Use-cases with map values
   }
% \end{wrapfigure}
\end{figure}



==> figures/pagerank-exectime.tex <==
\begin{wrapfigure}[17]{R}{{0.45\linewidth}  }
\centering
\begin{subfigure}{0.49\textwidth}  
\centering
\resizebox{.75\textwidth}{!}{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\Huge]
\begin{axis}[
    style=thick,
    height=6cm, 
    ymin=80, ymax=140, 
    width=12cm,
    xmin = 0,
    xmax = 10,
    bar width = 6pt,
    ylabel={\fontsize{20}{18} \selectfont Normalized Exec. \\ time (\%)}, 
    ylabel style={align=center, at={(-0.08,0.5)}},
    xtick={1.25,3.75,6.25,8.75},
    xticklabels={\textbf{Ligra},\textbf{Grid}\\ \textbf{Graph},\textbf{Gemini},\textbf{PG}\\ \textbf{Pull},\textbf{PG}\\ \textbf{Pull}},
    x tick label style={yshift=6.1cm, align=center},
    ytick style={draw=none},
    ymajorgrids=true, 
    grid style=dashed, 
    ytick={80,100,120}, 
    ytick style={draw=none},
    xtick style={draw=none},
    label style={font=\Huge}, 
    title style={font=\Huge},
]

%points in order: Ligra - GridGraph - Gemini - PowerGraph push - PowerGraph pull

%points for journal 0.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=amethyst,
    ybar,
    ] 
    coordinates { 
        (.5, 100)(3, 0)(5.5,96)(8, 100)
    }; 

%points for twitterwww 1+2.5x = i  
\addplot[ 
    color=black, 
    fill=aureolin,
    ybar,
    ] 
    coordinates { 
       (1, 104)(3.5, 0)(6,100)(8.5, 107)
    }; 
   
%points for twittermpi 1.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=persianred,
    ybar,
    ] 
    coordinates { 
        (1.5, 102)(4, 0)(6.5,102)(9,101)
    }; 
   
   
%points for friendster 2+2.5x = i  
\addplot[ 
    color=black,  
    fill=parisgreen,
    ybar,
    ] 
    coordinates { 
        (2, 0)(4.5, 0)(7,100)(9.5, 101)
    };  
 
   

\draw[dashed] (25,0) -- (25,2000);
\draw[dashed] (50,0) -- (50,2000);
\draw[dashed] (75,0) -- (75,2000);
\draw[dashed] (100,0) -- (100,2000);


\end{axis}
\end{tikzpicture}
}
\caption{Normalized execution time in seconds}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}  
\centering
\resizebox{.75\textwidth}{!}{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\Huge]
\begin{axis}[
    style=thick,
    height=6cm, 
    ymin=80, ymax=120, 
    width=12cm,
    xmin = 0,
    xmax = 10,
    bar width = 6pt,
    ylabel={\fontsize{20}{18} \selectfont Normalized \# of \\ edge ops (\%)}, 
    ylabel style={align=center, at={(-0.08,0.5)}},
    xtick={1.25,3.75,6.25,8.75},
    xticklabels={\textbf{Ligra},\textbf{Grid}\\ \textbf{Graph},\textbf{Gemini},\textbf{PG}\\ \textbf{Pull},\textbf{PG}\\ \textbf{Pull}},
    x tick label style={yshift=6.1cm, align=center},
    ytick style={draw=none},
    ymajorgrids=true, 
    grid style=dashed, 
    ytick={80,90,100,110,120}, 
    ytick style={draw=none},
    xtick style={draw=none},
    label style={font=\Huge}, 
    title style={font=\Huge},
]

%points in order: Ligra - GridGraph - Gemini - PowerGraph push - PowerGraph pull

%points for journal 0.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=amethyst,
    ybar,
    ] 
    coordinates { 
        (.5, 100)(3, 100)(5.5,100)(8, 100)
    }; 

%points for twitterwww 1+2.5x = i  
\addplot[ 
    color=black, 
    fill=aureolin,
    ybar,
    ] 
    coordinates { 
       (1, 100)(3.5, 100)(6,100)(8.5, 100)
    }; 
   
%points for twittermpi 1.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=persianred,
    ybar,
    ] 
    coordinates { 
        (1.5, 100)(4, 100)(6.5,100)(9,100)
    }; 
   
   
%points for friendster 2+2.5x = i  
\addplot[ 
    color=black,  
    fill=parisgreen,
    ybar,
    ] 
    coordinates { 
        (2, 0)(4.5, 100)(7,100)(9.5, 100)
    };  
 
   

\draw[dashed] (25,0) -- (25,2000);
\draw[dashed] (50,0) -- (50,2000);
\draw[dashed] (75,0) -- (75,2000);
\draw[dashed] (100,0) -- (100,2000);


\end{axis}
\end{tikzpicture}
}
\caption{Normalized number of edges processed}
\end{subfigure}
\caption{PageRank use-case.
\label{figure:pr-exec}}
\end{wrapfigure}




==> figures/streaming-exectime.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{0.49\textwidth}  
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\Huge]
\begin{axis}[
    style=thick,
    height=6cm, 
    ymin=80, ymax=120, 
    width=14cm,
    xmin = 0,
    xmax = 7.5,
    bar width = 6pt,
    ylabel={\fontsize{20}{18} \selectfont Normalized Exec. \\ time (\%)}, 
    ylabel style={align=center, at={(-0.08,0.5)}},
    xtick={1.25,3.75,6.25},
    xticklabels={\textbf{1k},\textbf{10k},\textbf{100k}},
    x tick label style={yshift=5.3cm, align=center},
    ytick style={draw=none},
    ymajorgrids=true, 
    grid style=dashed, 
    ytick={80,90,100,110,120}, 
    ytick style={draw=none},
    xtick style={draw=none},
    label style={font=\Huge}, 
    title style={font=\Huge},
]

%points in order: 1K - 10K - 100K

%points for journal 0.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=amethyst,
    ybar,
    ] 
    coordinates { 
        (.5, 103)(3, 102)(5.5,96)
    }; 

%points for twitterwww 1+2.5x = i  
\addplot[ 
    color=black, 
    fill=aureolin,
    ybar,
    ] 
    coordinates { 
       (1, 116)(3.5, 97)(6,102)
    }; 
   
%points for twittermpi 1.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=persianred,
    ybar,
    ] 
    coordinates { 
        (1.5, 101)(4, 101)(6.5,106)
    }; 
   
   
%points for friendster 2+2.5x = i  
\addplot[ 
    color=black,  
    fill=parisgreen,
    ybar,
    ] 
    coordinates { 
        (2, 100)(4.5, 104)(7,90)
    };  
 
   

\draw[dashed] (250,0) -- (250,2000);
\draw[dashed] (500,0) -- (500,2000);
%\draw[dashed] (75,0) -- (75,2000);
%\draw[dashed] (100,0) -- (100,2000);


\end{axis}
\end{tikzpicture}
}
\caption{$\SSSP$}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}  
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\Huge]
\begin{axis}[
    style=thick,
    height=6cm, 
    ymin=80, ymax=120, 
    width=14cm,
    xmin = 0,
    xmax = 7.5,
    bar width = 6pt,
    ylabel={\fontsize{20}{18} \selectfont Normalized Exec. \\ time (\%)}, 
    ylabel style={align=center, at={(-0.08,0.5)}},
    xtick={1.25,3.75,6.25},
    xticklabels={\textbf{1k},\textbf{10k},\textbf{100k}},
    x tick label style={yshift=5.3cm, align=center},
    ytick style={draw=none},
    ymajorgrids=true, 
    grid style=dashed, 
    ytick={80,90,100,110,120}, 
    ytick style={draw=none},
    xtick style={draw=none},
    label style={font=\Huge}, 
    title style={font=\Huge},
]

%points in order: 1K - 10K - 100K

%points for journal 0.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=amethyst,
    ybar,
    ] 
    coordinates { 
        (.5, 111)(3, 104)(5.5,93)
    }; 

%points for twitterwww 1+2.5x = i  
\addplot[ 
    color=black, 
    fill=aureolin,
    ybar,
    ] 
    coordinates { 
       (1, 100)(3.5, 102)(6,94)
    }; 
   
%points for twittermpi 1.5+2.5x = i  
\addplot[ 
    color=black, 
    fill=persianred,
    ybar,
    ] 
    coordinates { 
        (1.5, 85)(4, 98)(6.5,84)
    }; 
   
   
%points for friendster 2+2.5x = i  
\addplot[ 
    color=black,  
    fill=parisgreen,
    ybar,
    ] 
    coordinates { 
        (2, 94)(4.5, 90)(7,90)
    };  
 
   

\draw[dashed] (250,0) -- (250,2000);
\draw[dashed] (500,0) -- (500,2000);
%\draw[dashed] (75,0) -- (75,2000);
%\draw[dashed] (100,0) -- (100,2000);


\end{axis}
\end{tikzpicture}
}
\caption{$\CC$}
\end{subfigure}
\caption{Normalized execution time of the handwritten implementation in KickStarter framework with respect to the synthesized version in the $\name$ for a) $\SSSP$ and b) $\CC$ use-cases on dynamic input graphs with 1k, 10k and 100k edge mutations.
\label{figure:stream-exec}}
\end{figure*}




==> implementationfull.tex <==
\clearpage
\section{Implementation}
\label{sec-implementation-all}
\input{mappingframeworksfull}
\subsection{Path-based Reduction Synthesis}

\begin{figure}[H]
\begin{minipage}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
//NWR usecase
struct VValueType{
	uint32_t first;
	uint32_t second;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first < c.first) {
			w.first = b.first;
		} else {
			if (b.first > c.first) {
				w.first = c.first;
			}

		}if (b.second > c.second) {
			w.second = b.second;

		} else {
			if (b.second < c.second) {
				w.second = c.second;
			}
		}
	} while(((b.second > c.second ||
	 	b.first < c.first) &&
	    !(r=cas(a,c,w))));
	return r;
}
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
//Radius usecase
struct VValueType{
	uint32_t first;
	uint32_t second;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first < c.first) {
			w.first = b.first;
		} else {
			if (b.first > c.first) {
				w.first = c.first;
			}
		}if (b.second < c.second) {
			w.second = b.second;
		} else {
			if (b.second > c.second) {
				w.second = c.second;
			}
		}
	} while(((b.second < c.second ||
	    b.first < c.first) &&
	    !(r=cas(a,c,w))));
	return r;
}
\end{lstlisting}
\end{minipage}
\caption{Generated atomic reduce functions for more elaborate use-cases. 
The rule \irule{FMPair} is used to generate 
atomic reduce functions for NWR and Radius use-cases, respectively. \label{atomic-reduce}}
\end{minipage}
\end{figure}

\begin{figure}[ht!]
\begin{minipage}{1\textwidth}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
//BFS usecase
struct VValueType{
	uint32_t first;
	uint32_t second;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first < c.first) {
			w.first = b.first;
			w.second = b.second;
		} else {
			if (b.first > c.first) {
				w.first = c.first;
				w.second = c.second;
			}
		}
	} while((b.first < c.first && 
		!(r=cas(a,c,w)))); return r;
}

//CC usecase
struct VValueType{
	uint32_t first;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first > c.first) {
			w.first = b.first;
		} else {
			if (b.first < c.first) {
				w.first = c.first;
			}
		}
	} while((b.first > c.first && 
		!(r=cas(a,c,w)))); return r;
}

\end{lstlisting}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}
//SP usecase
struct VValueType{
	uint32_t first;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first < c.first) {
			w.first = b.first;
		} else {
			if (b.first > c.first) {
				w.first = c.first;
			}
		}
	} while((b.first < c.first &&
		!(r=cas(a,c,w)))); return r;
}

//WP usecase
struct VValueType{
	uint32_t first;
};
VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first > c.first) {
			w.first = b.first;
		} else {
			if (b.first < c.first) {
				w.first = c.first;
			}
		}
	} while((b.first > c.first && 
		!(r=cas(a,c,w)))); return r;
}

\end{lstlisting}
\end{minipage}
\caption{Generated atomic reduce functions for simple use-cases. \label{atomic-reduce} }
% For BFS use-case the reduce function is generated using \irule{FMRed}
\end{minipage}
\end{figure}
\clearpage
\begin{figure}[ht!]
\begin{minipage}{.5\textwidth}
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}
//WSP usecase
struct VValueType{
	uint32_t first;
	uint32_t second;
};

VValueType reduce(const VValueType a, 
		const VValueType b) {
	bool r = 0;
	VValueType c;
	VValueType w;
	do {
		c = a;
		w = c;
		if (b.first < c.first) {
			w.first = b.first;
			w.second = b.second;
		} else {
			if (b.first > c.first) {
				w.first = c.first;
				w.second = c.second;
			}

		}if (c.first == b.first) {
			w.first = c.first;
			w.second = std::max(b.second, c.second);
		}

	} while(((b.first < c.first ||
		 (c.first == b.first &&
		 b.second > c.second)) &&
		 !(r=cas(a,c,w))));
	return r;
}

\end{lstlisting}
\end{minipage}
\caption{Generated atomic reduce function for WSP usecase. 
The rule \irule{FPNest} is used to generate 
atomic reduce functions for WSP usecase. \label{atomic-reduce}}
\end{minipage}
\end{figure}



% \clearpage
% \subsection{Scalability}
% Three of the studied frameworks, GridGraph, Ligra and GeminiGraph, all require the
% user to specify an atomic reduce function. In order 
% to update the value of the vertices, the reduce function must 
% atomically set the new value of the vertices. 
% However, atomic compare and swap primitive provided by the library .i.e; 
% $sync\_bool\_compare\_and\_swap(T^* \ ptr, T \ oldVal, T \ newVal)$
% only accepts memory locations up to 8 bytes long. 
% This led to the limitation of only having vertex values of size no more than 8 bytes (2 integers).
% One solution to this problem is to use atomic library provided by the standard c++ compiler. 
% Vertex values can be wrapped inside an atomic instance. 
% Later, when doing reduction, the atomic library provides $compare\_and\_exchange()$ functionality
% which atomically swaps two atomic memory locations.
% Although this solution uses standard c++ functionality, 
% it does not scale very well. Our experiments showed that
% using $compare\_and\_exchange()$ does not scale after 20 bytes memory sizes and
% the performance drops drastically.
% To overcome these limitation, instead of 
% checking the contents of the memory and swapping memory contents,
% we indirectly swap the pointers to the memory locations.
% Since the size of the pointer in 32-bits and 64-bits architectures are 4 and 8 bytes 
% long, $sync\_bool\_compare\_and\_swap$
% builtin function can be used safely.
% 
% \begin{wrapfigure}[14]{R}{.5\textwidth}
% \begin{lstlisting}
%     bool reduce(VValue** val, VValue gatherVal) {
%         bool r;
%         VValue* oldVal;
%         VValue* newVal;     
%         do{
%             oldVal = *val;
%             newVal = calculateNewValue(val, gatherVal);
%         } while(!(r = cas(val, oldVal, newVal)));
%         
%         return r;
%     }
% \end{lstlisting}
% \caption{Reduce Function Template\label{reduce-func}. The cas function stands for
% sync\_bool\_compare\_and\_swap builtin.}
% \end{wrapfigure}
% 
% Lock-free synchronizations and data structures are known 
% to suffer from ABA problem.
% it occurs when a memory location is read twice 
% and compared and the comparison is is used to decides whether another thread has 
% updated the memory location meanwhile.
% If values are the same, the algorithm concludes that the
% no other thread have concurrently accessed and updated the memory location.
% However, comparing the contents of the memory location is not sufficient to 
% determine concurrent access.
% Consider the following scenario: 
% Thread $t_1$ reads the pointer to the value of the vertex, $p$.
% Concurrently, 
% Thread $t_2$ successfully swaps the pointer of the vertex to a new memory location $p'$.
% Thread $t_3$ also successfully swap the pointer of the same vertex with the same pointer $p$ to a new memory location.
% Thread $t_1$ continues and compares the pointer that it has read, $p$.
% Since pointers are the same, $t_1$ concludes that no concurrent update has happened sine 
% the first read, which is wrong.
% 
% We have resolved the ABA problem with tagged pointers. In modern architectures, each pointer only uses the last 48 bits of the whole 64 bits of the pointer. This gives us the 
% possibility to tag each pointer with an integer stored in the left most 16 bits.
% To indicate that the pointer have modified by other threads, the tag is increment.
% Thus, the compare and swap fails although the pointers are the same.
 
 

